Online Meta-Learning For Hybrid Model-Based Deep Receivers

Recent years have witnessed growing interest in the application of deep neural networks (DNNs) for receiver design, which can potentially be applied in complex environments without relying on knowledge of the channel model. However, the dynamic nature of communication channels often leads to rapid distribution shifts, which may require periodically retraining. This paper formulates a data-efficient two-stage training method that facilitates rapid online adaptation. Our training mechanism uses a predictive meta-learning scheme to train rapidly from data corresponding to both current and past channel realizations. Our method is applicable to any deep neural network (DNN)-based receiver, and does not require transmission of new pilot data for training. To illustrate the proposed approach, we study DNN-aided receivers that utilize an interpretable model-based architecture, and introduce a modular training strategy based on predictive meta-learning. We demonstrate our techniques in simulations on a synthetic linear channel, a synthetic non-linear channel, and a COST 2100 channel. Our results demonstrate that the proposed online training scheme allows receivers to outperform previous techniques based on self-supervision and joint-learning by a margin of up to 2.5 dB in coded bit error rate in rapidly-varying scenarios.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> sections_v0/abstract.tex <==
\begin{abstract} 
Many emerging digital communication applications will be required to operate in dynamic and complex environments. Recent years have witnessed a growing interest in the application of deep neural networks (DNNs) for receiver design, which can potentially be in complex environments without relying on knowledge of channel model and its parameters. However, the dynamic nature of communication channels often leads to rapid distribution shifts. In order to track temporal variations, DNN-based receivers may be required to periodically retrain in an efficient manner without inducing substantial overhead. 
%	
This paper formulates a data-efficient two-stage training method that facilitates rapid online adaptation of DNN-based receivers. First, our training mechanism proposes a predictive meta-learning scheme to learn to train rapidly from both local and global variations. As a second stage, we leverage on the explainable structure of model-based symbol detectors, training only specific sub-blocks of the model. The latter, referred to as modular training, is combined with predictive meta-learning method to assist in the quick adaption of the receiver to rapidly-varying channels.
Our extensive numerical results demonstrate that receivers combined with the novel algorithms outperform previous  approaches by a margin of up to 1.5dB in coded bit error rate over various challenging scenarios.
\end{abstract}

==> sections_v0/conclusion.tex <==
\section{Conclusions}
	\label{sec:Conclusions}
	\vspace{-0.1cm}
We proposed an online meta-learning algorithm for training data-driven receivers. Our approach aids the the receiver in tracking channel variations, incorporating both short-term and long-term relations. We combine three key ingredients that enable the tracking of rapidly time-varying channels: a model-based \ac{dnn} architecture; an online adaptation scheme with optimized initial weights; and the use of coded blocks for self-supervised training. Furthermore, We introduced a modular training scheme,  that exploits the interpretable structure of model-based detectors to aid in quick adaption to rapidly-varying channels. Numerical study demonstrates that, by properly integrating these methods, model-based receivers trained with the meta-training algorithm and modular training are capable of outperforming joint and online training approaches and are better able to track changing channels.

==> sections_v0/introduction.tex <==
\section{Introduction}
\vspace{-0.1cm} 
	
% Paragraph - need to operate in complex channel conditions
Traditional receiver design is dominated by methods that are based on statistical models. Such conventional receivers rely on  mathematical models that describe the transmission process, signal propagation, interference, and many other components of the system that affect the end-to-end communications. These statistical models typically adopt simplifying assumptions 
that make them tractable and understandable, and use parameters that vary over time as the channel conditions change.   The need to possess an accurate and simplified model may constitute a notable limitation in future communication technologies.  As high frequency bands and spectrum sharing  become widespread, current simplified models used for the channel, interference, and noise may be inaccurate \cite{xia2020mimo}. Moreover, emerging antenna architectures result in complex modelling of the transmission and reception process \cite{shlezinger2020dynamic}, while the deployment of intelligent surfaces notably complicates channel estimation \cite{alexandropoulos2021hybrid}. Furthermore, signalling in high frequencies is often prone to hardware non-idealities affecting the overall model, either unintentional or due to using limited hardware, e.g., few-bit \acp{adc} \cite{shlezinger2018asymptotic} and non-linear amplifiers \cite{singya17PA}.  This makes conventional channel-model-based techniques significantly more complex.
	
% Paragraph - deep learning for receivers
An alternative data-driven approach is based on deep learning. 
Deep learning systems have demonstrated unprecedented success in various applications, ranging from computer vision to natural language processing, and recently also digital communications and receiver design \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, oshea2017introduction}. While traditional receiver algorithms are channel-model-based, %relying on mathematical modeling of the signal transmission, propagation, and reception, 
\acp{dnn} are model-agnostic, and are trained from data. \ac{dnn}-aided receivers can operate efficiently in scenarios where the  channel model is unknown, highly complex, or difficult to optimize for~\cite{farsad2018neural}.

% Paragraph - inherent challenge due to temporal variations
Despite their potential in implementing digital receivers \cite{shlezinger2020inference,farsad2020data}, deep learning solutions are subject to several challenges that limit their applicability in important communication scenarios. A fundamental difference between digital communications and traditional deep learning applications stems from the dynamic nature of communication systems, and particularly of wireless channels.  \acp{dnn} consist of highly-parameterized models that can represent a broad range of mappings. As such, massive data	sets are typically required to learn a desirable mapping.  The dynamic nature of communication channels implies that the statistical model can change considerably over time, and thus a \ac{dnn} trained for a given channel may no longer perform well on future channel realizations. %\ac{dnn}-aided receivers are thus likely to require frequent retraining, at the cost of degraded spectral efficiency due to pilot transmissions. % which adds to the increased computational burden involved in training \acp{dnn}.

To apply \ac{dnn}-aided transceivers in time-varying channels, two main approaches are considered in the literature. The first  attempts to learn a single mapping that is applicable to a broad range of channel conditions. This class of methods includes the straightforward approach of training a \ac{dnn} using data corresponding to an extensive set of expected channel conditions, which is referred to as {\em joint learning}\cite{oshea2017introduction, xia2020note}. An additional related method trains in advance a different network for each expected channel, and combines them as a deep ensemble \cite{raviv2020data}. However, these strategies typically require a large amount of training data, and  deviating from the training setup, i.e., operating in a channel whose characteristics differ from those observed during training, can greatly harm performance \cite{park2020learning}. 

The alternative strategy is to track the channel variations. This can be achieved by providing the \ac{dnn} with a model-based channel estimate \cite{he2020model,honkala2021deeprx,khani2020adaptive, samuel2019learning, goutay2021machine}. However,  channel estimation involves imposing a relatively simple model on the channel, typically a linear Gaussian model, which may be inaccurate in some setups. 
When operating without channel knowledge, tracking the channel involves periodically retraining the network. To provide data for retraining, one must either transmit frequent pilots, or, alternatively, use decoded data for training. Such self-supervised training can be implemented by either using successfully decoded \ac{fec} codewords, as  in \cite{shlezinger2019viterbinet, teng2020syndrome}, or  by providing a measure of confidence per each symbol and selecting those with the highest confidence for retraining, as proposed in \cite{sun2020generative}. Nonetheless,  the volumes of data one can obtain in real-time, either from pilots or from decoded transmissions, are limited and are not at the scale of typical data sets used for training \acp{dnn}. Retrained \ac{dnn}-aided receivers should thus utilize compact \ac{dnn} architectures. This can be achieved without compromising accuracy by using hybrid model-based/data-driven receivers that incorporate domain knowledge. Following this principle, data-driven implementations of the Viterbi scheme \cite{viterbi1967error},  BCJR method \cite{bahl1974optimal}, and  iterative \ac{sic}  \cite{choi2000iterative} were proposed in \cite{shlezinger2019viterbinet,shlezinger2020data, shlezinger2019deepSIC}, respectively. Yet, even with compact architectures, relatively large data sets are still required and typical \ac{dnn} training procedures are likely to induce non-negligible delay. 

The ability to retrain quickly is highly dependent on the selection of a suitable initialization of the iterative training algorithm. While the common strategy is to use random weights, the work \cite{shlezinger2019viterbinet} used the previous learned weights as an initial point for  retraining. 
An alternative approach is to optimize the initial point via meta-learning \cite{park2020meta,simeone2020learning,jiang2019mind,park2020learning}. Following this approach, one not only retrains, but also optimizes the hyperparameters that dictate the retraining process. In particular, it was shown in \cite{park2020learning} that by optimizing the initial weights, rather than using random weights or the previous ones, the receiver can quickly adapt to varying channel conditions. 
%Furthermore, to enable online training in a self-supervised manner, it was proposed in \cite{shlezinger2019viterbinet} to exploit the presence of \ac{fec} codes, commonly utilized in digital communications, to retrain in a decision-directed fashion.


In this work we propose an online training algorithm to enable rapid adaptation of channel-model-agnostic \ac{dnn}-aided receivers from scarce pilots. Our algorithm considers both long and short term variations in the channel: We choose the initial weights by a communication-adapted meta-learning \cite{finn2017model} novel algorithm, which we enhance to facilitate training for future (predicted) channel realizations, while tracking local variations in a self-supervised manner. The latter is achieved by exploiting the presence of \ac{fec} codes, commonly utilized in digital communications, to retrain in a decision-directed  fashion as in \cite{shlezinger2019viterbinet,teng2020syndrome}.
Additionally, we exploit the explainable structure of model-based receivers \cite{shlezinger2020model} to re-train only specific parts of the model. This new approach to online training, referred to as \textit{modular training}, enables adaption in quickly-changing scenarios as one has to train fewer parameters. 

% to train This enabling the use of self-generated labels that extend the availability of supervised data beyond the pilot blocks. 
Our main contributions are summarized as follows:
\begin{itemize}
    \item \textbf{Predictive online meta-learning training algorithm -} We tailor the \ac{maml} method \cite{finn2017model} to incorporate temporal evolution exhibited by time-varying channels.
    Specifically, we modify the support and query tasks, such that a small number of gradient updates, calculated by training on the last decoded block, will minimize the loss (or error) on the next (predicted) data block. 
    \item \textbf{Modular training of interpretable architectures -} 
    The interpretable nature of hybrid model-based data-driven receivers implies that their neural building blocks often have a concrete operational meaning, such as the detection of the transmissions of a specific user in a multi-user network. We propose to leverage this interpretablity to retaining only specific subsets of the architecture in the presence of temporal variation patterns often exhibited in wireless communications, e.g., those arising due to mobility of some of the users.
    
    \item \textbf{Extensive Experimentation -} We extensively evaluate the proposed training scheme for both \ac{siso} and \ac{mimo} systems, considering three different time-varying channel profiles: Linear synthetic channel, a non-linear synthetic channel, and a COST 2100 \cite{liu2012cost}  channel.
    We show gains of up to 1.5dB in coded \ac{ber}, compared to joint and online approaches, over a set of challenging channels.
\end{itemize}

 The rest of this paper is organized as follows:  Section~\ref{sec:Model} details the system model, while Section~\ref{sec:Hybrid Meta-Learning for Data-Driven Receivers} presents the meta-learning algorithm. In Section~\ref{sec:modular-training} we dive into model-based receivers and how should one exploit their interpretable structure via modular training. Finally, experimental results and concluding remarks are presented in Section~\ref{sec:Simulation} and Section~\ref{sec:Conclusions}, respectively.

Throughout the paper, we use boldface letters for vectors, e.g., ${\myVec{x}}$; $({\myVec{x}})_i$ denotes
the $i$th element of ${\myVec{x}}$. %We use upper-case letters for \acp{rv}, and lower-case letters for deterministic quantities. 
Calligraphic letters, such as $\mySet{X}$, are used for sets, 
and $\mySet{R}$ is the set of real numbers.



==> sections_v0/method.tex <==
\section{Predictive Online Meta-Learning for DNN-Aided Receivers}
	\label{sec:Hybrid Meta-Learning for Data-Driven Receivers}
	\vspace{-0.1cm}
	In this section we study parameters' adaption of a generic \ac{dnn}-aided receiver $\Weights$ to continuously maintain low error rates in time-varying channels. Modification of these weights involves training, which requires the receiver to have access to data, i.e., pairs of transmitted blocks and their observed channel outputs corresponding to the channel input-output relationship. This gives rise to two core challenges: First, while one can use pilot transmissions from data, the time-varying nature of the channel implies that  pilot-based data is likely to not represent the underlying channel conditions for some or all of the data blocks. In addition, even if one can extract labeled training data online, i.e., from blocks containing information messages, when the channel varies quickly, i.e., the coherence block $\Blklen$ is relatively short, the amounts of data corresponding to the instantaneous channel may be limited. Combining this with the typical lengthy duration of \ac{dnn} training procedures makes online adaptation of \ac{dnn}-aided receivers a challenging task. 
	
	These challenges are tackled by our predictive online meta-training algorithm. To describe this algorithm, we begin with introducing self-supervised training in Subsection~\ref{subsec:Online}, describing how can one train online without pilots in slow-fading channels. Next, we present our proposed method in Subsection~\ref{subsec:high-level}, which allows online training to be carried out over rapidly time-varying channels. We then discuss the resulting algorithm in Subsection~\ref{subsec:MetaLearningDiscussion}.

%-----------------------------------
%	Decision-Directed Online Training
%-----------------------------------
\vspace{-0.2cm}
\subsection{Self-Supervised Online Training}
\label{subsec:Online}
\vspace{-0.1cm} 

% \textcolor{red}{At this point in the paper we have already formulated the channel model and the problem. So now we need to gradually lead towards our solution based on the model. So I recommend starting the section by:\\
% Start by explaining that since we consider the operation of \ac{dnn}-aided receivers in complex channels, as detailed in Subsection~\ref{subsec:Channel}, one would need to periodically re-train the \ac{dnn} in order to preserve reliable operation in time-varying conditions. \\
% Then, explain that the core algorithmic challenge in doing so stems from the availability of data. Training requires data corresponding to the instantaneous channel conditions being observed currently, while the generic protocol detailed in Subsection-??? implies that pilots, which can be used to formulate a labeled training set, are scarce and may not correspond to the current channel. }

% We regard the problem of \ac{dnn}-aided receivers in complex time-varying channels, as detailed in Subsection~\ref{subsec:Channel}, where the distribution of the channel output $\myY$ changes with time. As the deviation between the trained-on channel and the tested one increases, one obviously needs to periodically re-train the receiver to preserve high performance operation. 

The first part of our online adaptation mechanism is based on self-supervision, i.e., the extraction of training data from information-bearing blocks. Our self-supervision technique follows the approach used  \cite{shlezinger2019viterbinet} for exploiting the presence of channel coding to re-use confident decisions by re-encoding a successfully decoded word and using it for online training. 
%
Following this approach, the parameters of a \ac{dnn}-aided receiver are adapted on a block by block basis; That is, on any incoming block $\myVec{y}_j$. Even if the deep symbol detector is not trained for the instantaneous channel realization from which $\myVec{y}_j$ is generated and thus its estimate $\hat{\myVec{s}}_j$ may differ from the true transmitted symbol vector, the \ac{fec} decoder can still correct these errors, as long as they are within the Hamming distance of the code. Specifically, the channel decoder takes as input the estimated block $\hat{\myVec{s}}_j$, and outputs a decoded message along with the number of errors, as an indication of the correctness of its decoded message. When decoding is correct, i.e. the number of errors is 0, the decoded and demodulated message $\hat{\myVec{m}}_j$ is encoded and modulated into the estimated transmitted symbols  $\myVec{s}_j$.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/self-supervised online training figure.png}
    \vspace{-0.6cm}
    \caption{Self-supervised online training based on channel coding.}
    \label{fig:self-supervised training}
\end{figure}
	

% \textcolor{red}{We can consider adding a figure visualizing how online training operates. It can be divided into two parts - symbol detection and online training. }

Specifically, the detector for the $j$th block is parameterized by the weight vector $\Weights_j$, which is applied to $\myVec{y}_j$. When decoding is successful, one can confidently generate a data pair $\{\myVec{s}_{j}, \myVec{y}_{j}\}$ to be used for training the parameters for the next block, i.e., generate $\Weights_{j+1}$. Since symbol detection can be treated a classification task, this is achieved by minimizing the empirical cross entropy loss:
\begin{align}
\label{eq:meta_1}
  \mathop{\arg \min}_{\Weights} \left\{ \mySet{L}_{j}(\Weights) = -\sum_{i=1}^{\Blklen}\log \hat{P}_{\Weights}\left(\myVec{y}_{i,j}|\myStateR_{i,j} \right)\right\}.
\end{align}
 The expression $\hat{P}_{\Weights}\left( \myVec{y}  |  \myStateR\right)$ is the soft output of the \ac{dnn}-aided receiver corresponding to $\myStateR$ when applied to the data block $ \myVec{y}$. The optimization problem in \eqref{eq:meta_1} is approximately solved using gradient-based optimization i.e., through $I$ iterations of the form
 \begin{align}
\label{eq:local_update}
\Weights_{j+1}^{(t+1)} = \Weights_{j+1}^{(t)} - \eta \nabla_{\Weights}\mySet{L}_{j}(\Weights_{j+1}^{(t)}),
 \end{align}
 where $\eta > 0$ is the learning rate. The computation of the gradient steps requires some initial setting, i.e., $\Weights_{j+1}^{(0)}$ should be set to some vector, which is a hyperparameter of the training procedure. We henceforth denote this hyperparameter vector used for self-supervised training of $\Weights_{j+1}$ as  $\HyperParams_{j+1}$, i.e., $\Weights_{j+1}^{(0)} = \HyperParams_{j+1}$. 
 The computation of the gradient in \eqref{eq:local_update} is typically approximated via random sampling among available $B$ symbols within the block to implement \ac{sgd} and its variants, typically used for training DNNs \cite[Ch. 4]{goodfellow2016deep}.  The online training scheme is presented in Fig.~\ref{fig:self-supervised training}.

%In order to enable an adaptation mechanism, the receiver maintains at each block index $j$ a vector of hyperparameters $\HyperParams_j$. %\NirCmt{Do we need to introduce the data buffer at this stage? We do not really use it here, but for meta-learning. So I guess the main question is whether the purpose of this section is to discuss how online self-supervised training is done in the literature, or to explain how we do it here? If we go with the latter, we need to explain that the proposed scheme only observes short-term variations, i.e., those between the current block and the next one, and thus missing out on long-term variation, such as patterns of variations observed in the past. To be able to also account for these longer variations, we save decisions in the buffer, whose usage is revealed in ths sequel.}.

%At each data block $j$, given the initialization hyperparameter vector\NirCmt{Perhaps we should not state here how the initial hyperparameters vector is set, just say that we use some initialization $\HyperParams_j$. Then, when we conclude the section say that the approach used in \cite{shlezinger2019viterbinet} used $\HyperParams_j=\Weights_{j-1}$, which implies that only short-term variations are accounted for in the training procedure, as both the data and the optimization hyperparameters correspond to the current instantaneous channel realization.} $\HyperParams_j$ and successfully decoded blocks' pair $\{\myVec{s}_{j-1}, \myVec{y}_{j-1}\}$, the algorithm updates the model parameters vector $\Weights_j$. 
 
 For reliable operation, the self-supervision training algorithm relies on two main characteristics of digital communications over time-varying channels: 
  \begin{enumerate}
    \item The first is the presence of \ac{fec} coding that provides a safe margin and allowing one to recover the transmitted symbols even as a small number of errors occur. The exact number is dependent on the Hamming distance of the \ac{fec} code. Moreover, one can identify when re-encoding is possible, employing the re-encoded block for training. 
    
    \item The second property exploited is the fact that dynamic channels are of continuous nature; Thus one can reasonably assume that the data from the channel observed in the $j$th time index is still applicable to the $j+1$th channel realization. Following this line of reasoning, the researchers in  \cite{shlezinger2019viterbinet} used $\HyperParams_{j+1}=\Weights_{j}$. 
 \end{enumerate}
 
While the first point is a must-have for any training algorithm, as it depends on correctly labeled samples, we claim that the second point is inadequate for tracking fast-varying channels and should be revised. As the instantaneous channel conditions change and the data distribution varies quickly, the \ac{fec} mechanism fails. Adapting locally in a self-supervised manner by setting the hyperparamters $\HyperParams_{j+1}=\Weights_{j}$ accounts for only short term variations, as both the data and the optimization hyperparameters correspond to the current instantaneous channel realization. In order to train effectively from short blocks in complex channels, we propose to incorporate long term relations by altering the setting of the hyperparameters $\HyperParams_{j+1}$.  
 
 %mini-batch. Note  \eqref{eq:local_update} describes a single \ac{sgd} iteration,  multiple iterations are similarly accommodated.

% \textcolor{red}{I recommend concluding the above paragraph by clarifying that the ability to carry out such self-supervision relies on two characteristics of digital communications over time-varying channels: The first is the presence of coding, which allows one to recover re-form the transmitted symbols even when detection has errors as long as these errors are below the Hamming distance of the \ac{fec} code, as well as identify when such re-encoding is possible due to error detection codes. The second property exploited is the fact that dynamic channels are not arbitrarily time-varying, and thus one can train using data corresponding the channel observed during the $j$th while still being applicable in the $j+1$th channel realization. \\
% After saying that, please explain why is this not enough on its own. This will lead us to the need optimize the hyperparameters $\theta_j$ in order to effective online training from short blocks and with few epochs, which is discussed in the following section. This way you lead your readers through your method (which on its own is quite complicated, thus requires a gradual gentle well-motivated introduction of its components). }


%-----------------------------------
%	High-Level Description
%-----------------------------------
\vspace{-0.2cm}
\subsection{Predictive Online Meta-Learning} 
\label{subsec:high-level}
\vspace{-0.1cm}
While online training is successful when the channel variations are relatively slow, i.e., the block size $\Blklen$ is large enough to allow the aggregation of sufficient self-supervised data, it may fail to track fast changing channels. To tackle this, we exploit long-term memory, i.e., previously observed channel variation patterns, using the meta-learning approach, in contrast to the self-supervised learning which exploits short-term memory. Meta-learning, often referred to as {\em 'learning to learn'} \cite{lemke2015metalearning}, focuses on optimizing the hyperparamters, i.e., parameters which dictate the learning algorithm, rather than being learned by it. In conventional non-meta-learned systems, these hyperparamters, also referred to as inductive bias, are handcrafted by human designers, typically based on abstract guidelines and experience. 
 Meta-learning enables the learning of these parameters  without relying on heuristics.


Our meta-training algorithm operates without explicit knowledge of the channel input-output relationship \eqref{eqn:ChModel1}, apart from its memory $L$ and its coherence time duration $\Blklen$. 
Following the  \ac{maml} framework of \cite{finn2017model}, we use data to optimize the hyperparameter vector $\HyperParams_j$, which determines the initialization used to update the detector's parameters $\Weights_{j+1}$ based on the data of block $j$ via, e.g., \ac{sgd}. Specifically, we use long-term variations in the channel to determine an initialization for the self-supervised online training algorithm (Subsection~\ref{subsec:Online}). This is done by modifying \ac{maml} such that the support task is set to the {\em detection of the current block}; while the query task, for which the parameters should adapt, is the {\em detection of the next block}. This allows us to account for the predictive nature of self-supervised online training, where data from the current block is used to train for the subsequent (predicted) channel realization. Incorporating patterns in the channel variations, observed in past blocks, into the predictive detection aids to minimize the overall \ac{ber}.

% \textcolor{red}{Conclude this section by revealing the rationale of our approach to the readers (before digging into the details. This includes two important aspects of our algorithm: \\
% First, that instead of directly applying conventional \ac{maml}, as done in \cite{park2020learning}, we modify its operation to account for the predictive nature of self-supervised online training, where data from the current block is used to train for the subsequent (predicted) channel realization.   \\
% Second, that we use long-term variations in the channel to determine an initialization for the training algorithms which is expected to facilitate rapid training based on channel variation patters between subsequent blocks observed in the past.} 
	
	
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/FlowChart3.png}
    \caption{Illustration of the operation of the proposed meta-training algorithm.}
    \label{fig:FlowChart1}
\end{figure}
	
In particular, upon the reception of a block of channel outputs $\myVec{y}_j$, the method operates in three stages, illustrated as a block diagram in Fig.~\ref{fig:FlowChart1}:
\begin{enumerate}
    \item \emph{Detection}: Each incoming data block $\myVec{y}_j$ is mapped into an estimated symbol block $\hat{\myVec{s}}_j$, with the mapping determined by the current parameters vector $\Weights_{j}$. Then, it is decoded by using an \ac{fec} decoder to produce the demodulated and decoded message $\hat{\myVec{m}}_j$. When decoding is correct, as determined by error detection, the message $\hat{\myVec{m}}_j$ is re-encoded and modulated, producing an estimated transmitted vector $\tilde{\myVec{s}}_j$. This block is inserted along with its observations $\myVec{y}_j$ into a labelled buffer $\mathcal{D}_{j}$.  This buffer contains pairs of previously received blocks $\myVec{y}_j$ along with their corresponding transmitted signal $\myVec{s}_j$, or an estimated version thereof. The buffer $\mathcal{D}_j$ contains $D$ such pairs, and is managed in a first-in-first-out mode. A pilot block $(\myVec{s}_j, \myVec{y}_j)$ is directly inserted into  $\mathcal{D}_{j}$ upon reception.
    \item \emph{Online training}: In each data block $j$, if decoding is successful, the weights $\Weights_{j+1}$ are updated by using the hyperparameters $\HyperParams_{j+1}$ and the newly decoded block $(\myVec{s}_{j}, \myVec{y}_{j})$, as detailed in Subsection~\ref{subsec:Online}. Otherwise, no update is carried out. A similar update takes place for pilot block $j$ with pilot block $(\myVec{s}_j, \myVec{y}_j)$.
    \item \emph{Predictive meta-learning}: The hyperparameter {$\HyperParams_{j+1}$} is optimized so as to enable fast and efficient adaptation of the model parameter $\Weights_{j+1}$ based on the last successfully decoded block $(\myVec{s}_{j}, {\myVec{y}}_{j})$ using \eqref{eq:local_update}. Adopting MAML \cite{finn2017model}, we leverage the data in the buffer $\mathcal{D}_j$ by considering the problem
    %\NirCmt{I think that the indexing in \eqref{eq:meta_2} is confusing and inconsistent. I think it should be $ \HyperParams_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}(\Weights =  \HyperParams  -  \kappa \nabla_{\HyperParams}\mySet{L}_{j'}(\HyperParams))$. Can you please double check?}:
    %
\begin{align}
    \label{eq:meta_2}
      \HyperParams_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}(\Weights =  \HyperParams  -  \kappa \nabla_{\Weights }\mySet{L}_{j'}(\HyperParams)),
\end{align}
% %
% \begin{align}
%     \label{eq:meta_2}
%       \HyperParams_{j +1}  =  \mathop{\arg \min}_{\HyperParams}     \sum_{\{\myVec{s}_{j+1}, {\myVec{y}}_{j +1}\} \in \mathcal{D}_j}     \mySet{L}_{j +1}(\Weights_{j+1} =  \HyperParams  -  \kappa \nabla_{\HyperParams}\mySet{L}_{j}(\HyperParams)),
% \end{align}
where $\kappa >0$ is the meta-learning rate. The parameters $\Weights$ in \eqref{eq:meta_2} follow the same update rule in \eqref{eq:local_update} by using the last available block $(\myVec{s}_{j'}, \myVec{y}_{j'})$ in the buffer  prior to index $j'+1$. Furthermore, in line with \eqref{eq:meta_1}, the loss $\mySet{L}_{j'+1}(\Weights)$ is computed based on data from the {\em following} available block $(\myVec{s}_{j'+1}, \myVec{y}_{j'+1})$. When the buffer $\mathcal{D}_j$ contains a sufficiently diverse set of pairs of subsequent past channel realizations, the hyperparameter obtained via \eqref{eq:meta_2} should facilitate fast training for future channels via \eqref{eq:local_update} \cite{park2020end}. 
\end{enumerate} 

The online-meta training is applied periodically, i.e., once every $F$ blocks. Moreover, if $\Weights_j$ and/or $\HyperParams_j$ are not updated in a given block index $j$, they are preserved for the next block by setting  $\Weights_{j+1} = \Weights_j$ and/or $\HyperParams_{j+1}=\HyperParams_j$.
%
The online adaptation framework %is detailed in the sequel, and 
is summarized in Algorithm~\ref{alg:online-meta-learning}.


\begin{algorithm} %!
\DontPrintSemicolon
\caption{Online Adaptation on Incoming Block $j$}
\label{alg:online-meta-learning}
\KwIn{Step sizes $\eta, \kappa$; number of iterations $I$; threshold $\epsilon$; buffer $\mathcal{D}_{j}$; hyperparameter $\HyperParams_{j}$}
\KwOut{Hyperparameter $\HyperParams_{j+1}$; weights $\Weights_{j+1}$; buffer $\mathcal{D}_{j+1}$}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
%{\bf Initialization} inductive bias $\HyperParams_1$ and ViterbiNet $\Weights_1$ \\
%{\bf Initialization} buffer $\mathcal{D}_1$ as empty, i.e., $\mathcal{D}_1 \leftarrow [ \hspace{0.2cm} ]$ \\
%\For{$j = 1,2,\ldots$}{
Receive ${\myVec{y}}_j$ 	\tcp*{received channel output}
\uIf{Pilot}{
$\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ \tcp*{known pilots} 
  }
  \Else{
  Equalize and decode ${\myVec{y}}_j$ into  $\hat{\myVec{m}}_j$ \tcp*{data}
  \uIf{Decoding is correct}{
  Modulate  $\hat{\myVec{m}}_j\mapsto\myVec{s}_j$ \; 
$\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ 
  }
%   \uElse{pass
%   }
  }
\nonl\texttt{Online predictive meta-learning (every $F$ blocks)}\;
Set $\HyperParams_{j+1}^{(0)} = \HyperParams_j$\;
\For{$i=0,1,\ldots$}{
\label{stp:Random} Randomly select block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})\in \mathcal{D}_{j}$\; % except for the last block in the buffer $\mathcal{D}_j$\\  
      {\uIf{$(\myVec{s}_{j'}, {\myVec{y}}_{j'})\notin \mathcal{D}_{j}$}{
% pass;  
%   }
%   \uElse{
  go back to line \ref{stp:Random} \tcp*{invalid data for meta-learning}
  }
  }
  Set $\hat{\HyperParams}^{(0)} = \HyperParams_{j+1}^{(i)}$\;
    \For{$t=0,1,\ldots,I-1$}{
   Use block $(\myVec{s}_{j'}, {\myVec{y}}_{j'})$ to compute \tcp*{support task}
      \begin{equation*}
\hat{\Weights} = \hat{\HyperParams}^{(t)} -\eta\nabla_{\Weights} \mySet{L}_{j'}(\Weights=\hat{\HyperParams}^{(t)}). \end{equation*} \;
    Use subsequent block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})$ to update \tcp*{query task}
  \begin{equation*}
\hat{\HyperParams}^{(t+1)} = \hat{\HyperParams}^{(t)} - \kappa \nabla_{\Weights}\mySet{L}_{j'+1}(\Weights =\hat{\Weights}). 
\end{equation*}
    }
    Update hyperparameter as $\HyperParams_{j+1}^{(i+1)} =\hat{\HyperParams}^{(I)}$ \tcp*{meta-update}
% Update the parameters with $I$ iterations on the selected block $(\myVec{s}_{j'}, {\myVec{y}}_{j'})$ via \eqref{eq:local_update} as %\tcp*{local update}
%   \begin{equation*}
% \hat{\Weights}_{j+1} = \HyperParams_{j+1}^{(i)}-\eta\nabla_{\HyperParams_{j+1}^{(i)}} \mySet{L}_{j}(\HyperParams_{j+1}^{(i)}). \end{equation*} \;
% Evaluate loss at block $j+1$% $\hat{\Weights}_{j+1}$ for block $j+1$ computed as
% , $\mySet{L}_{j+1}(\hat{\Weights}_{j+1})$\;
% Update hyperparameter $\HyperParams_{j+1}$ via \tcp*{meta-update}
%   \begin{equation*}
% \HyperParams_{j+1}^{(i+1)} = \HyperParams_{j+1}^{(i)} - \kappa \nabla_{\HyperParams_{j+1}^{(i)}}\mySet{L}_{j+1}(\hat{\Weights}_{j+1}). 
% \end{equation*}
}
Set hyperparameter $\HyperParams_{j+1} =\HyperParams_{j+1}^{(i+1)}$ \;
\nonl\texttt{Online learning (on each block)} \;
{\uIf{(Pilot) or (Decoding is correct)}{
\label{stp:onlineStart}
 Train $\Weights_{j+1}$ with $({\myVec{s}}_j, {\myVec{y}}_j)$ and initialization $\HyperParams_{j+1}$  via \eqref{eq:meta_1} \tcp*{update} 
  }
  \Else{ 
      $\Weights_{j+1} \leftarrow \Weights_j$ \tcp*{no update}
  }
  \label{stp:onlineEnd}$\mathcal{D}_{j+1}\leftarrow \mathcal{D}_{j}$ \tcp*{keep buffer}
  }
 %}
\end{algorithm}

% TODO NIR CONTINUE FROM HERE 13-Dec
%-----------------------------------
%	Discussion
%-----------------------------------
\vspace{-0.2cm}
\subsection{Discussion} 
\label{subsec:MetaLearningDiscussion}
\vspace{-0.1cm}
Algorithm~\ref{alg:online-meta-learning} is designed to enable rapid online training from scarce pilots by simultaneously accounting for short-term variations, via online training, as well as long-term variations, using the proposed predictive meta-learning. Compared to joint learning, which uses many channel realizations to train the parameters of the models, we adapt the hyperparamters, i.e. the initial weights, based on actual realization observed after deployment. In particular, we build upon the insight that while past realizations are likely to differ from the current channel and thus may not contribute to training the \ac{dnn} weights, they often represent how the channel tends to vary between blocks. Hence, by tuning the initial weights based on past channel variations, the detector learns how the channel varies over a long history. This improves self-supervised online training as in \cite{shlezinger2019viterbinet}, which employs learning using a single block, i.e., only building upon the fact that the subsequent channel is expected to bear some similarity to the current one, without accounting for temporal variation patterns observed in the past. Algorithm~\ref{alg:online-meta-learning} learns to predict the channel coefficients based on the sequential transmission, allowing the receiver to train accurately from small data sets and achieve improved performance over rapidly time-varying channels. Our experimental results reported in Section~\ref{sec:Simulation} show that the proposed method achieves an improvement of up to 1.5dB in coded \ac{ber} over a range of SNRs and scenarios.  %That is, our proposed training procedure is designed to exploit long-term domain knowledge, from both the channel and the transmission model. 

The gain associated with  Algorithm~\ref{alg:online-meta-learning} come at the cost of additional complexity, as our proposed approach is more computational demanding compared with offline joint learning or online training without meta-learning. The excessive complexity can be controlled by, e.g., modifying the number of meta-learning iterations $I$ and/or changing the meta-learning frequency $F$. One can also consider gradually adjusting these key parameters over time, balancing the excessive computational burden based on the current load, mobility level, and power conditions. Furthermore, the rapid growth and expected proliferation of dedicated hardware accelerators for deep learning applications \cite{chen2019deep} indicates that the  number of hardware-capable digital communication devices will increase. Such devices are expected to be able to carry out the needed computations associated with online meta-learning in run-time.

The usage of meta-learning techniques to facilitate \ac{dnn}-aided communications in time varying channels was also considered in the recent literature in \cite{yuan2020transfer,zhang2021embedding, wang2021jointly, jung2021meta}, with its application for the adaptation of deep receivers  studied in \cite{park2020learning, cohen2021learning}. 
%Considering related works, paper \cite{park2020learning} focuses on an IoT scenario, where a meta-learning scheme is devised to aid a black-box demodulator in quick adaptation to new end-to-end channel conditions from few pilots. 
Though sharing the meta-learning concept, our proposed algorithm fundamentally differs from these previous works is several core aspects: First, \cite{park2020learning,cohen2021learning} focused on communication where on each coherence duration, i.e. for each channel realization, a relatively large number of pilots are transmitted along with the data symbols, and these pilots are used for learning purposes. %Hence, \cite{park2020learning} considering only joint training, and not self-supervised training, as training was carried out based on pilots and data the have undergone the same channel. 
This %implies that the approach in \cite{park2020learning} 
is suitable for relatively slow variations, where devoting a sufficient portion of each block to pilots is plausible. Our proposed approach does not share this limitation due to its incorporation of self-supervised training and the proposed predictive meta-learning. In fact, Algorithm~\ref{alg:online-meta-learning} can be applied in a setup where only some initial pilots are transmitted, followed by a long pilot-free horizon, thus communicating in a highly spectrally efficient manner. 
Furthermore, while \cite{park2020learning,cohen2021learning} considered black-box architectures, we also show how our training algorithm can benefit from utilizing interpretable model-based architectures. This capability is enabled by the incorporation of modular training, presented in the following section. % Section~\ref{sec:modular-training}.%\NirCmt{I am not sure that this description properly captures the distinction from \cite{park2020learning}. You should clarify that while the usage of meta-learning for enabling fast adaptation was considered in \cite{park2020learning}, our proposed adaptation differs from that in \cite{park2020learning} is several core aspects: First, \cite{park2020learning} focused on communication where on each coherence duration, i.e., on each channel realization, a relatively large number of pilots is transmitted followed by data symbols. Hence, \cite{park2020learning} did not consider any form of self-supervision, as training was carried out based on pilots, and both pilots and data have undergone the same channel. This implies that the approach in \cite{park2020learning} is suitable for relatively slow variations, where devoting a sufficient portion of each block to pilots does not substantially limit the spectral efficiency. Our proposed approach does not share this limitation due to its incorporation of self-supervised training and predictive meta-learning. In fact, Algorithm~\ref{alg:online-meta-learning} can be applied in a setup where only some initial pilots are transmitted, followed by a long pilot-free horizon, thus communicating in a highly spectrally efficient manner. Finally, while \cite{park2020learning} considered black-box architectures, we also show how our training algorithm can benefit from utilizing interpretable model-based architectures, as we discuss in Section~\ref{sec:modular-training}.}  . 


% \textcolor{red}{Important items to discuss:\\
% 1. Capitalize on the difference from joint learning  -- they use many past channel realizations (and typically simulated channels) to train the parameters of the deep model, we use them to adapt the {\em hyperparamters}, i.e., the optimizer, based on actual realization observed after deployment. The model itself is still adapted to the current instantaneous channel, while past data is used to optimize the optimizers. \\
% 2. We have to discuss complexity. This will inevidably arise from the reviewers and is indeed a challenge associated with our proposed design. We need to clarify that the method we propose allows DNN-aided receivers to track rapidly time-varying channels, and that these additional training rounds may be computationally complex to carry out in some applications. However, we can emphasize that the rapid growth and expected proliferation of dedicated hardware accelerators for deep learning applications, combined with the fact that training procedures are naturally prone to parallelization, indicates that more and more future digital communication devices are expected to be equipped with hardware capabilities allowing to carry out such computations in run-time.   }

==> sections_v0/model_based_detectors.tex <==
\section{Modular Training}
\label{sec:modular-training}
The training algorithm detailed in Section~\ref{sec:Hybrid Meta-Learning for Data-Driven Receivers} is agnostic of the \ac{dnn} architecture; It is applicable to any deep receiver parameterized by $\Weights$. Nonetheless, it is preferable to combine it with architectures that not highly-parameterized, since such \acp{dnn} can be trained with relatively small data sets. An emerging approach to realize reliable receivers which utilize compact \acp{dnn} is to design them in a hybrid model-based/data-driven fashion \cite{farsad2021data, balatsoukas2019deep}, integrating the available knowledge of the desirable algorithmic steps into the receiver architecture in a principled manner. 
The  interpretable architecture of hybrid model-based/data-driven receivers brings forth an additional benefit exploited by our training algorithm, which is the ability to leverage domain knowledge to train only sub-blocks of the overall \ac{dnn} online via {\em modular training}.



% This Section explores the notion of modular training: How can one exploit domain knowledge to accelerate the adaptive training of \ac{dnn}-aided receivers in rapidly-varying channels?

% \subsection{Model-Based Detectors}
% \label{subsec:model-based}

\subsection{Modular Online Training of Model-Based Deep Receivers}
\label{subsubsec:modular_training}
Model-based deep learning refers to a family of techniques for designing systems which combine principled model-based algorithms with data-driven deep learning techniques \cite{shlezinger2020model}. Hybrid design techniques, such as deep unfolding \cite{monga2021algorithm}, neural augmentation \cite{satorras2020neural}, and \ac{dnn}-aided algorithms \cite{farsad2021data}, gave rise to a multitude of deep receiver architectures, including, e.g., \cite{shlezinger2020data,samuel2019learning,he2020model,nachmani2018deep,balatsoukas2019deep, be2019active,shlezinger2019deepSIC, shlezinger2019viterbinet}. Hybrid  model-based/data-driven receivers build on existing communication models and incorporate deep learning into their design, rather than replace the known model altogether. These receivers can be agnostic to the channel-model, imitating the operation of a suitable detection algorithm without relying on knowledge of the actual channel model and its parameters. Moreover, they are much more compact in terms of parameters, thus are faster to train and require fewer training samples to reach convergence.







% \textcolor{red}{The following paragraph should be revised in light of its purpose. Our goal here is to provide a generic description of the idea of modular training, and in the next subsection exemplify it for modular training of DeepSIC. We need to highlight to the findings upon which this approach relies:\\
% 1. Hybrid model-based/data-driven receivers (don't refer to them as model based receivers as this term is likely to be mistaken with classical ones) often employ interpretable architectures. Interperability here is in the sense that one can often relate their internal features with an operational quantity, and affiliate their intermediate sub-blocks with concrete tasks that arise from the operation of the model-based algorithm from which they originate. \\
% 2. While communication channels are time-varying, it is not rare that one can relate the variations to a specific component in the channel. For instance, in multi-user communications involving both static and mobile users, channel variations are often due to the movement of the mobile users. Alternatively, channel variations can also be due to users joining or leaving the network. \\
% The next thing to do is to say that modular training seeks to jointly exploit these findings, for setups where the interpretable nature of the deep receiver sub-blocks can be related with the components of the channel where variations originate. Then explain how this done from a relatively broad perspective. Only then proceed into the example of modular training of DeepSIC provided in the following section. }

Our motivation is to exploit the structure of the hybrid model-based/data-driven receivers in order to quickly adapt to new environments. We highlight the two main pillars of our method:
\begin{enumerate}
    \item Hybrid receivers often employ \textit{interpretable architectures} which carry out a principled algorithm in a learned fashion. Their interpretability means that one can often relate their internal features with an operational quantity: Each sub-block is responsible for a concrete task that arises from the operation of the model-based algorithm. 
    \item Often in communications scenarios, one can relate the channel variations to specific component in the setup. For  instance,  in  multi-user  communications  involving both  static  and  mobile  users,  channel  variations  are  often  due  to  the  movement  of  the  mobile users. Alternatively, channel variations can also be due to users joining or leaving the network. These variations, being invariant to how the receiver operates, have a great impact on the system and should be taken into consideration.
\end{enumerate}
Our approach, coined modular training, seeks to jointly exploit these properties for  setups  where  the  interpretable  nature  of  the  deep  receiver  sub-blocks  can  be  related  with the  components  of  the  channel  where  variations  originate. Specifically, as hybrid model-based/data-driven receivers can often divided into meaningful sub-blocks, we wish to train only those that relate to a specific time-varying component of the underlying channel. We next show how to apply modular training in uplink \ac{mimo} systems, employing the DeepSIC receiver \cite{shlezinger2019deepSIC}.


\subsection{Modular DeepSIC for Tracking Mobile Users}
\label{subsec:DeepSIC}
Here, we provide an example for online modular training of \ac{dnn}-aided receivers. To that aim, we begin by describing the considered scenario of uplink multi-user \ac{mimo} with both mobile and static users. Then, we describe the hybrid model-based/data-driven architecture used, which is DeepSIC proposed in \cite{shlezinger2019deepSIC}. Finally, we show how the knowledge on the nature of the variations combined with the interpretable architecture of DeepSIC gives rise to efficient online adaptation via modular training, and provide a discussion.

\subsubsection{Uplink Multi-User \ac{mimo}}
We consider an uplink mobile multi-user \ac{mimo} settings. This is a special case of the generic  model detailed in Subsection~\ref{subsec:Channel}, where the channel is memoryless ($L=1$) while the receiver has $N>1$ antennas and it communicates with $K>1$ users. Some of users with indexes $k\in \mathcal{K}\subset\{1,\ldots,K\}$ are mobile while the remaining are static. We further focus on a case where the receiver knows which of the users are mobile, i.e., it has prior knowledge of $\mathcal{K}$. For example, such scenario arises in a traffic monitoring infrastructure, when a multi-antenna \ac{bs} communicates with both static road-side units, which are known to be static, as well as with mobile vehicles.

%-----------------------------------
%	DeepSIC
%-----------------------------------
\subsubsection{DeepSIC Receiver}
Next, we describe the receiver chosen to highlight the benefits of modular training. The iterative  \ac{sic} algorithm proposed in \cite{choi2000iterative} is a \ac{mimo}  detection method that combines multi-stage interference cancellation with soft decisions. For brevity, we omit here the subscripts representing the time instance and the block index, using $\myVec{Y}$ to denote the random channel output and $\myVec{S}=[S_1,\ldots,S_K]^T$ as the transmitted symbols. 
This algorithm operates in $Q$ iterations, refining an estimate of the conditional \acl{pmf} of $S_k$, denoted by $\hat{\myVec{p}}_{k}^{(q)}$ where $q$ denotes the iteration number. This estimate   is generated for every symbol $k \in \{1,2,\ldots, K\}$ using the corresponding estimates of the interfering symbols $\{S_l\}_{l \neq k}$ obtained in the previous iteration $\{\hat{\myVec{p}}_{\tilde{k}}^{(q-1)}\}_{\tilde{k}\neq k}$. Iteratively repeating this procedure refines the conditional distribution estimates, allowing the detector to accurately recover each symbol from the output of the last iteration.  This iterative procedure is illustrated in Fig.~\ref{fig:SoftIC}(a). 

\begin{figure}
	\centering
	\includegraphics[width = \columnwidth]{fig/DeepSIC1.png}
	\vspace{-0.4cm}
	\caption{(a) Iterative soft interference cancellation, and (b) the \ac{dnn}-aided DeepSIC.}
	%	\vspace{-0.4cm}
	\label{fig:SoftIC}
\end{figure}

The hybrid data-driven/model-based  DeepSIC \cite{shlezinger2019deepSIC} is a DNN-aided architecture that learns to implement the iterative SIC method from data. This is achieved by replacing the interference cancellation and soft decoding steps with trainable classifiers, i.e., parameterizing the classic building blocks with \acp{dnn}, each with parameters denoted by $\Weights^{k,q}$. The set $\{\Weights^{k,q}\}$ stands for the entire model's parameters $\Weights = \{\Weights^{k,q}\}$. The resulting \ac{dnn}-aided receiver, illustrated in Fig.~\ref{fig:SoftIC}(b), was shown in \cite{shlezinger2019deepSIC}  to be able to carry out \ac{sic}-based \ac{mimo} detection in complex channel models where the model-based algorithm is inapplicable. 

\subsubsection{Modular Training of DeepSIC}
While DeepSIC is comprised of an interconnection of classification \acp{dnn}, its hybrid model-based/data-driven operation allows to identify the operational meaning of its internal features. In particular, the output of the \ac{dnn} with weights $\Weights^{k,q}$ is a soft estimate of the symbol of the $k$th user, and thus the channel relating this user and the receiver is encapsulated in the parameters $\{\Weights^{k,q}\}_{q=1}^Q$. 

Modular training exploits this ability to relate specific sub-blocks with different users. It replaces the online training part in steps \ref{stp:onlineStart}-\ref{stp:onlineEnd} of Algorithm~\ref{alg:online-meta-learning}. Let us assume that a single $k$th user is moving. Then, one can use the self-supervised data acquired online and the meta-optimized hyperparameters to train only the part of the model that depends on the moving user. In our case, this  is attributed sub-block \acp{dnn} $\{\Weights^{k,q}\}_{q=1}^Q$. In particular, when the receiver knows that the $k$th user is moving during the $j$th data block, it can apply Algorithm~\ref{alg:online-meta-learning} to optimize the hyperparameters while only adjusting the weights $\{\Weights^{k,q}\}_{q=1}^Q$. The resulting modular training is summarized as  Algorithm~\ref{alg:modular-training}. 

\begin{algorithm} %!
\DontPrintSemicolon
\caption{Online Modular Training for DeepSIC (Steps \ref{stp:onlineStart}-\ref{stp:onlineEnd} of Algorithm~\ref{alg:online-meta-learning})}
\label{alg:modular-training}
\KwIn{Moving users $\mySet{K}$; parameters $\Weights_j$; hyperparameters $\HyperParams_{j+1}$; block data $({\myVec{s}}_j, {\myVec{y}}_j)$.}
\KwOut{Parameters $\Weights_{j+1}$.}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
\uIf{(Pilot) or (Decoding is correct)}{ 
 Use $({\myVec{s}}_j, {\myVec{y}}_j)$ and initialization $\HyperParams_{j+1}$ to train only $\{\Weights_{j+1}^{k,q}\}_{q=1}^Q$, $k\in\mathcal{K}$ \tcp*{update} 
  Set $\Weights_{j+1}^{k,q} = \Weights_{j}^{k,q}$, for each $k\notin\mathcal{K}$
  }
  \Else{ 
      $\Weights_{j+1} \leftarrow \Weights_j$ \tcp*{no update}
  }
% %{\bf Initialization} inductive bias $\HyperParams_1$ and ViterbiNet $\Weights_1$ \\
% %{\bf Initialization} buffer $\mathcal{D}_1$ as empty, i.e., $\mathcal{D}_1 \leftarrow [ \hspace{0.2cm} ]$ \\
% %\For{$j = 1,2,\ldots$}{
% Receive ${\myVec{y}}_j$ 	\tcp*{received channel output}
% \uIf{Pilot}{
% $\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ \tcp*{known pilots} 
%   }
%   \Else{
%   Equalize and decode ${\myVec{y}}_j$ into  $\hat{\myVec{m}}_j$ \tcp*{data}
%   \uIf{Decoding is correct}{
%   Modulate  $\hat{\myVec{m}}_j\mapsto\myVec{s}_j$ \; 
% $\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ 
%   }
% %   \uElse{pass
% %   }
%   }
% Generate an initial guess of the conditional distributions $\{\hat{\myVec{p}}_k^{(0)}\}_{k=1}^K$. \;
% \For{$q=1,\ldots,Q$}{
% \nonl\texttt{Training is based on Algorithm~\ref{alg:online-meta-learning} or self-supervised learning in Subsection~\ref{subsec:Online}. \;}
% Train $\HyperParams_{j}^{k,q}$ with ${\myVec{y}}_j$ and $\{\hat{\myVec{p}}_{\tilde{k}}^{(q-1)}\}_{\tilde{k}\neq k}$ \tcp*{update only $k^{th}$ user}
% Compute the probabilities $\{\hat{\myVec{p}}_k^{(q)}\}_{k=1}^K$
% }
\end{algorithm}

% \textcolor{red}{The description of this subsection misses on what we are trying to show. I suggest we proceed along with the formula provided in the previous section - what is the architecture, what are the type of channel variations considered, and how does modular training operate. More precisely, here is how I think you should structure it: \\
% 1. Start by saying that here, we provide an example for online modular training of \ac{dnn}-aided receivers. To that aim, we begin by describing the considered scenario, which is an uplink multi-user \ac{mimo} channel with mobility. Then, we describe the hybrid model-based/data-driven architecture used, which is DeepSIC proposed in \cite{shlezinger2019deepSIC}, after which we show how the knowledge of the nature of the variations combined with interpretable architecture of DeepSIC gives rise to efficient online adaptation via modular training.\\
% 2. Dedicate a paragraph to considered channel. Clarify that we are focusing on a memoryless uplink multi-user \ac{mimo} channel, and show how it is a special case of the generic channel model you give in Section~\ref{sec:Model}. Explain what is the prior knowledge about the nature of variations that you posses, and say that represents setups where some of the users known to be mobile while the remaining ones are known to be static. You can give an example a traffic monitoring infrastructure where a multi-antenna \ac{bs} communicates with both static road-side units as well as mobile vehicles.  \\
% 3. Only then go into the architecture of DeepSIC. A paragraph like you have here is enough but please read it along with the overall section and make sure that it fits into the story in a coherent manner and that the notations are indeed in line with those used for formulating the channel. \\
% 4. Now explain how modular training takes place. First describe in words, then summarize it as an algorithm. \\
% 5. Conclude with a discussion - begin by capitalizing on the benefits, which is mostly due to the fact that you only a train a portion of the overall network dictated by the ratio of the mobile users to the overall users in the network. Clarify that our numerical results presented in Section~\ref{sec:Simulation} demonstrate that the proposed approach translated the prior knowledge of the nature of the variations into improved performance, particularly when dealing with short blocks, i.e., short coherence duration of rapidly varying channels. Then, go into the downsides. First, clarify that while we are training only the models corresponding to the mobile users, it is expected that these variations may also affect how the decisions for the static users are carried out. Emphasize that this can be resolved by also including some training rounds for the overall network, using the modular training as a warm start for accelerating training, yet in our numerical study we clearly observe that mere modular training yields improved performance over using the data to train the overall network. You can also say that this approach clearly relies on prior knowledge of which users are mobile, and that we leave the study of its resilience to inaccuracies in this domain knowledge for future work. Feel free to add any more items you think should be discussed.
% }



\subsubsection{Discussion}
\label{subsec:modular-training-discussion}
Modular training algorithm exploits the model-based structure of hybrid \ac{dnn} receivers to further accelerate the training on short blocks and improve adaptation. This follows from the fact that Algorithm~\ref{alg:modular-training} trains online only  a  portion  of  the  overall  network, i.e., it uses the same data as in Algorithm~\ref{alg:online-meta-learning} while adapting less parameters, thus gaining in convergence speed and accuracy of the trained model. The exact portion of the overall parameters is  dictated  by  the  ratio  of  the mobile users to the overall users in the network. The smaller the ratio is, the more one can benefit from modular training. We validate the benefits of modular training in Subsection~\ref{subsec:modular-training} and show that this approach can decrease the average \ac{ber} significantly. Indeed, our experimental results demonstrate that the proposed approach successfully translates the prior knowledge on the nature of  the  variations  into  improved  performance,  particularly  when  dealing  with  short  blocks,  i.e. short coherence duration of rapidly varying channels. 

Algorithm~\ref{alg:modular-training} can be viewed as a form of transfer learning, as it trains online only parts of the parameters. Yet, it is specifically tailored towards interpretable architectures, adapting internal sub-modules of the overall network, as opposed to the common transfer learning approach of retraining the output layers. In particular, while the formulation of Algorithm~\ref{alg:modular-training} jointly trains the sub-modules associated with all mobile users, one may train them separately in an iterative fashion, and even sequentially train modules associated with different iteration, building upon the fact that each module $\Weights^{k,q}$ should produce a soft estimate of $S_k$.  Modular training can also be enhanced to carry out some final tuning of the overall network since, e.g., the channels of the mobile users is expected to also affect how their interference is canceled when recovering the remaining users via the sub-modules which are not adapted online.  
Finally, it is noted that Algorithm~\ref{alg:modular-training} relies on knowledge of the mobile users, and thus incorrect knowledge of $\mathcal{K}$ is expected to affect the accuracy of the trained receiver.  We  leave  the  study  of  the resilience of modular training and the aforementioned extensions for future work.

==> sections_v0/results.tex <==
\section{Numerical Evaluations}
\label{sec:Simulation}
\vspace{-0.1cm} 
In this section we numerically evaluate the proposed online adaptation scheme in finite-memory \ac{siso} chanels and in memorylesss multi-user \ac{mimo} setups\footnote{The source code used in our experiments is available at \href{https://github.com/tomerraviv95/MetaDeepSIC}{https://github.com/tomerraviv95/MetaDeepSIC}}. 
We first describe the receivers compared in our experimental study, detailing the architectures in Subsection~\ref{subsec:simEqualizers} and the training methods in Subsection~\ref{subbsec:Training Methods}. Then, we present the main simulations results on linear synthetic channels, non-linear synthetic channels, and channels obeying the COST 2100 model in Subsections~\ref{subsec:synth_simulation_results} to \ref{subsec:cost_simulation_results}. Finally, we numerically evaluates the combination of our online meta-learning method with the proposed modular training algorithm, as well as the effect of our learning schemes on pilot efficiency, in Subsections~\ref{subsec:modular-training} and \ref{subsec:pilot-training}, respectively.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_train_channel.png}
    \caption{Synthetic training channel.}
    \label{fig:synthetic_train_channel}
    \end{subfigure} 
    %
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_test_channel.png}
    \caption{Synthetic test channel.}
    \label{fig:synthetic_test_channel}
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/cost_channel.png}
    \caption{COST 2100 channel.}
    \label{fig:COSTChannel} 
    \end{subfigure}
    \caption{Examples of time-varying channels: channel coefficients versus block index.}
    \figSpace
    \label{fig:channels} 
    \vspace{-0.18cm}
\end{figure*}


%-----------------------------------
%	ViterbiNet
%-----------------------------------
% \subsection{ViterbiNet}
% \label{subsec:ViterbiNet}


% Following the channel definition of Subsection~\ref{subsec:SISOChannel}, the Viterbi equalizer solves the maximum likelihood sequence detection problem
% \begin{align}
% \hat{\myVec{s}}_j   
% &= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i,j}\right)\right\}.
% \label{eqn:ML3} 
% \end{align}	
% In particular,  \eqref{eqn:ML3} is solved recursively via dynamic programming, by  iteratively updating a {\em path cost} $c_i(\myStateR)$ for each state $\myStateR\in \bar{\mySet{S}}$ for $i=1,2,\ldots,B$. ViterbiNet implements Viterbi detection in a data-driven fashion by training a \ac{dnn} to provide a parametric estimate of the likelihood function $\hat{P}_{\Weights}\left( \myVec{y}  |  \myStateR\right)$. Meta-ViterbiNet \cite{raviv2021meta} applies Algorithm~\ref{alg:online-meta-learning} to ViterbiNet, leading to higher adaptivity over fast channel variations.

%-----------------------------------
%	Evaluated Equalizers
%-----------------------------------
\vspace{-0.4cm}
\subsection{Evaluated Receivers}
\label{subsec:simEqualizers}
The receiver algorithms used in our experimental study vary based on the considered settings, which are \ac{siso} channels with finite-memory and memoryless \ac{mimo} channels
\vspace{-0.1cm}
\subsubsection{\ac{siso} Finite-Memory Channels}
For the \ac{siso} setting, we compare two  \ac{dnn}-aided receivers:
\begin{itemize}
    \item The ViterbiNet equalizer, proposed in \cite{shlezinger2019viterbinet}, which is a hybrid model-based/data-driven implementation of the Viterbi detector for finite-memory channels of the form \eqref{eqn:ChModel1} \cite{viterbi1967error}. The Viterbi equalizer (from which ViterbiNet originates) solves the maximum likelihood sequence detection problem
\begin{align}
\hat{\myVec{s}}_j   
&= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i-\Mem+1,j},\ldots, \myStateR_{i,j}\right)\right\}.
\label{eqn:ML3} 
\end{align}	
    ViterbiNet computes each log likelihood using a trained \ac{dnn} that requires no prior knowledge of the channel conditional distributions $ \Pdf{\myVec{Y}_j |  \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}$. This internal \ac{dnn} is implemented using three fully-connected layers of sizes $1\times 100$, $100\times 50$, and $50 \times \CnstSize^\Mem$, with activation functions set to sigmoid (after first layer), ReLU (after second layer), and softmax output layer.
    %sigmoid and ReLU activations, respectively, and a softmax output layer. 
    \item A recurrent neural network  symbol detector, comprised of a sliding-window \ac{lstm} classifier with two hidden layers of 256 cells and window size $\Mem$, representing a black-box \ac{dnn} benchmark \cite{tandler2019recurrent}.
\end{itemize}

We also employ the Viterbi equalizer operating with complete knowledge of the channel as a baseline method.

\subsubsection{Memoryless \ac{mimo} Channels}
In our \ac{mimo} experiments, we evaluate two  \ac{dnn}-aided receivers:
\begin{itemize}
    \item The DeepSIC receiver detailed in Subsection~\ref{subsec:DeepSIC}. The building blocks of DeepSIC are implemented using three fully-connected layers:  An $(N + K - 1) \times 100$ first layer, a $100 \times 50$ second layer, and a $50 \times \CnstSize$ third layer, with a sigmoid and a ReLU intermediate activation functions, respectively. The number of iterations is set to $Q=5$.  
    %sigmoid and ReLU activations, respectively, and a softmax output layer. 
    \item A ResNet10 black-box neural network, which is based on the  DeepRX architecture proposed in \cite{honkala2021deeprx}. The architecture is comprised of 10 residual blocks \cite{he2016deep}, each block has two convolutional layers with 3x3 kernel, one pixel padding on both sides, and no bias terms, with a ReLU  in-between. 
    A 2D batch normalization follows each convolutional layer.
\end{itemize}

\subsection{Training Methods}
\label{subbsec:Training Methods}
Before the evaluation phase begins, we generate a set $\mathcal{D}_0$ of $T_p$ pilot blocks. We then use the following methods for adapting the deep receivers:
\begin{itemize}
    \item {\em Joint training}: The \ac{dnn} is  trained on $\mathcal{D}_0$ only by minimizing the empirical cross-entropy loss, and no additional training is done in the evaluation phase.
    \item {\em Online training} \cite{shlezinger2019viterbinet}: The \ac{dnn} is initially trained  on $\mathcal{D}_0$ by minimizing the empirical cross-entropy loss. Then, during evaluation, the \ac{dnn} parameters vector $\Weights_j$ is re-trained on each successfully decoded data block and on each incoming pilot block. Precisely, online training follows \eqref{eq:local_update} by using $\Weights_{j}$ in lieu of $\HyperParams_{j+1}$. %, using a fixed non-optimized inductive bias $\HyperParams$.
    \item {\em Online meta-learning}: 
    Here, we first meta-train $\HyperParams_0$ with $\mathcal{D}_0$ similar to \eqref{eq:meta_2} as
    \begin{align*}
    %\label{eq:offline_meta}
     \HyperParams_{0} = \mathop{\arg \min}_{\HyperParams} \sum_{\{(\myVec{s}_{ j'}, {\myVec{y}}_{ j'}), (\myVec{s}_{ j'+1}, {\myVec{y}}_{ j'+1})\} \in \mathcal{D}_0}    \mySet{L}_{ j'+1}(\Weights = \HyperParams  -  \kappa \nabla_{\Weights }\mySet{L}_{ j'}(\Weights =\HyperParams)).
\end{align*}
    
    %To this end, meta-training splits the buffer $\mathcal{D}_0$ into following-words pairs as $(\boldsymbol{y}^B_0,\boldsymbol{y}^B_1),\ldots,(\boldsymbol{y}^B_{T_t-2},\boldsymbol{y}^B_{T_t-1})$. The first word of each pair $\boldsymbol{y}^B_{2n}$ is used for the local update (\ref{eq:local_update}), while the second word $\boldsymbol{y}^B_{2n+1}$ is used for the global update calculation as in
	%\begin{align}
	%\label{eq:meta_2_pred_offline}
	 % \mathop{\arg \min}_{\HyperParams_0} \sum_{\text{odd }j} \mySet{L}_j(\Weights= \HyperParams_0 - \eta \nabla_{ \HyperParams_0}\mySet{L}_{j-1}( \HyperParams_0)).
	%\end{align}
	This  process yields the initial hyperparameters $\HyperParams_0$. 
	Then, during evaluation,   Algorithm~\ref{alg:online-meta-learning} is used with online learning every block and online meta-learning every $F=5$ blocks. The number of online meta-learning updates   equals that of online training, thus inducing a relative small overhead due to its additional computations. The combination of online meta-learning with ViterbiNet is henceforth referred to as {\em Meta-ViterbiNet}, while the DeepSIC receiver trained with this approach is coined {\em Meta-DeepSIC}.
\end{itemize}


%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{Linear Synthetic Channel Results}
\label{subsec:synth_simulation_results}
\vspace{-0.1cm}
We begin with evaluating the adaptation mechanisms on synthetic time-varying linear channels with additive Gaussian noise, considering both a finite-memory \ac{siso} setting as well as a memoryless \ac{mimo} setup.
%
\subsubsection{\ac{siso} Finite-Memory Channels} 
%We refer to the combination of the ViterbiNet equalizer and online meta-training as Meta-ViterbiNet. 
Recalling Figure \ref{fig:transmission}, we transmit $T_p=T_d=300$ blocks. The block length is set to $\Blklen = 136$ symbols, representing a relatively short coherence duration for the time-varying channel. Each block includes 120 information bits, encoded using a \acl{rs} [17,15] code with two parity symbols under \ac{bpsk} modulation, i.e., $\mySet{S} = \{\pm 1\}$.  %The online meta-learning in Algorithm \ref{alg:online-meta-learning} is executed every $K=5$ blocks. 

We consider a linear Gaussian channel, whose input-output relationship is given by
\begin{equation}
\label{eqn:Gaussian}
\myY_{i,j} = \sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j},
\end{equation}
where $\myVec{h}_j = [h_{0,j},\ldots,h_{\Mem-1,j}]^T$ are the real channel taps, and $w_{i,j}$ is \acl{awgn} with variance $\sigma^2$. We set channel memory to $\Mem = 4$ with the taps $\{h_{l,j}\}$ being generated using a synthetic model representing oscillations of varying frequencies. 
%
Here,  the signals received during the pilots used for initial training $(\mathcal{D}_0)$ are subject to the time-varying channel whose taps are illustrated in Fig.~\ref{fig:synthetic_train_channel}; while we use the taps illustrated in Fig.~\ref{fig:synthetic_test_channel} for testing. This channel presents oscillations of varying frequencies, where  the periods of the taps become aligned as the noise subsides. 

In Fig.~\ref{fig:SyntheticBERvsBlock} we plot the evolution of the average coded \ac{ber} of the considered receivers when the \ac{snr}, defined as $1/\sigma^2$, is set to $12$ dB. Fig.~\ref{fig:SyntheticBERvsBlock} shows that Meta-ViterbiNet significantly outperforms its benchmarks, demonstrating the gains of the proposed online meta-learning training and its suitability when combined with receiver architectures utilizing relatively compact \acp{dnn}. In particular, it is demonstrated that each of the ingredients combined in Meta-VitebiNet, i.e., its model-based architecture, the usage of self-supervision, and the incorporation of online meta-learning, facilitates operation in time-varying conditions: The ViterbiNet architecture consistently outperforms the black-box \ac{lstm} classifier; Online training yields reduced \ac{ber} as compared to joint learning; and its combination with meta-learning via Algorithm~\ref{alg:online-meta-learning} yields the lowest \ac{ber} values.  

To further validate that these gains also hold for different \acp{snr}, we show in Fig.~\ref{fig:SyntheticBERvsSNR} the average coded \ac{ber} of the evaluated receivers after 300 blocks, averaged over 5 trials. We observe in Fig.~\ref{fig:SyntheticBERvsSNR} that for \ac{snr} values larger than $8$ dB, Meta-ViterbiNet consistently achieves the lowest  \ac{ber} values among all considered data-driven receivers, with gains of up to 0.5dB over the online training counterpart.


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_block.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:SyntheticBERvsBlock}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_snr.png}
    \caption{Coded \ac{ber} after 300 blocks vs. SNR.}
    \label{fig:SyntheticBERvsSNR}
    \end{subfigure}
    %
    \caption{\ac{siso} synthetic linear Gaussian channel, $\Blklen = 136$.}
    \label{fig:SyntheticBER} 
    \figSpace
\end{figure*}



\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_block_mimo.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:SyntheticBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_snr_mimo.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:SyntheticBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} synthetic linear Gaussian channel, $\Blklen = 96$.}
    \label{fig:SyntheticBERMIMO} 
    \figSpace
\end{figure*}

\subsubsection{Memoryless MIMO Channels} 
For the \ac{mimo} setting, use $T_p=T_d=50$ blocks. The block length is set to $\Blklen = 96$ symbols, encoding 80 information bits with \acl{rs} [12,10] code. The input-output relationship of a the memoryless Gaussian \ac{mimo} channel is given by
\begin{equation}
\label{eqn:GaussianMIMO}
\myY = \myMat{H}\myS + \myVec{W},
\end{equation}
where $\myMat{H}$ is a known deterministic $N\times K$ channel matrix, and $\myVec{W}$ consists of $N$ i.i.d Gaussian \acp{rv}.  
We set the number of users and antennas $N=K=4$. The channel matrix $\myMat{H}$ models spatial exponential decay, and its entries are given by
$\left( \myMat{H}\right)_{n,k} = e^{-|n-k|}$, for each $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$.  The transmitted symbols are generated from a \ac{bpsk} constellation in a uniform i.i.d. manner, i.e., $\mathcal{S}=\{\pm 1\}$.

The numerical results for the memoryless Gaussian channel \eqref{eqn:GaussianMIMO} are depicted in Fig.~\ref{fig:SyntheticBERMIMO}.
Note that Fig.~\ref{fig:SyntheticBERvsBlockMIMO} shows the average coded \ac{ber} of the receivers for ${\rm SNR} = 14$ dB, while Fig.~\ref{fig:SyntheticBERvsSNRMIMO} shows a sweep over a range of \ac{snr} values after 50 blocks. Similarly to Meta-ViterbiNet in the finite-memory \ac{siso} setting, Meta-DeepSIC outperforms all other training methods in medium to high SNRs. Here, the black-box architectures perform quite poorly, unable to compete with the model-based architecture of DeepSIC due to short blocklengths and the highly limited volumes of data used for training. Training DeepSIC with Algorithm~\ref{alg:online-meta-learning} outperforms the joint training approach with gains of up to 0.5dB, and with gains of 1.5dB over online training, which notably struggles in tracking such rapidly time-varying and challenging conditions.


\vspace{-0.4cm}
\subsection{Non-Linear Synthetic Channel Results}
\label{subsec:syntNL_simulation_results}
\vspace{-0.1cm}
Next, we evaluate the proposed online meta-learning scheme in non-linear synthetic channels, where one can greatly benefit from the model-agnostic nature of \ac{dnn}-aided receivers. 

\subsubsection{\ac{siso} Finite-Memory Channels} To check the robustness of our method in a non-linear case, we generate a non-linear channel by applying a non-linear transformation to synthetic channel in \eqref{eqn:Gaussian}. The resulting finite-memory \ac{siso} channel is give by
\begin{equation}
\label{eqn:Gaussian1}
\myY_{i,j} =\tanh{\Big(C * \Big(\sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j}\Big)\Big)}.
\end{equation}
This operation may represent, e.g., non-linearities induced by the receiver acquisition hardware. The hyperparameter $C$ stands for a power attenuation at the receiver, and chosen empirically as $C=\frac{1}{2}$. All other hyperparameters and settings are the same as those used in the previous subsection. This simulation shows a consistent gain of around $0.75$dB over the SNRs with values of $8$dB - $12$dB, as observed in Fig.~\ref{fig:NonLinearSyntheticBERSISO}.

\subsubsection{Memoryless \ac{mimo} Channels} Similiarly to the \ac{siso} case, we simulate a non-linear \ac{mimo} channel from \eqref{eqn:GaussianMIMO} via
\begin{equation}
\label{eqn:Gaussian2}
\myY = \tanh{\Big(C *\Big(\myMat{H}\myS + \myVec{W}\Big)\Big)}.
\end{equation}
Similarly, $C=\frac{1}{2}$ and the remaining simulation settings are chosen as in Subsection~\ref{subsec:synth_simulation_results}. The numerical results for this channel are illustrated in Fig.~\ref{fig:NonLinearSyntheticBERMIMO}, showing that the superiority of our approach is maintained in non-linear setups. In particular, we note that gains of up to 0.5dB in high SNRs are achieved compared with joint learning, while online method is unable to track the channel and performs much worse. Here, our gain becomes apparent as the SNR increases.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_block_siso.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:NonLinearSyntheticBERvsBlockSISO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_snr_siso.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:NonLinearSyntheticBERvsSNRSISO}
    \end{subfigure}
    %
    \caption{\ac{siso} synthetic non-linear Gaussian channel, $\Blklen = 96$.}
    \label{fig:NonLinearSyntheticBERSISO} 
    \figSpace
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_block_mimo.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:NonLinearSyntheticBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_snr_mimo.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:NonLinearSyntheticBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} synthetic non-linear Gaussian channel, $\Blklen = 96$.}
    \label{fig:NonLinearSyntheticBERMIMO} 
    \figSpace
\end{figure*}

%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{COST 2100 Channel Results}
\label{subsec:cost_simulation_results}
\vspace{-0.1cm}

Next, we consider channels generated using the COST 2100 geometry-based stochastic channel model \cite{liu2012cost}. This model is widely used in indoor wireless communications.

% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/test_8x8_cost_ant1.png}
%     \caption{Antenna 1 channel.}
%     \label{fig:cost_channel_antenna1}
%     \end{subfigure}
%     %
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/test_8x8_cost_ant2.png}
%     \caption{Antenna 2 channel.}
%     \label{fig:cost_channel_antenna2}
%     \end{subfigure}
%     %
%     \caption{\ac{mimo} COST 2100 channels.}
%     \label{fig:CostBER} 
%     \figSpace
% \end{figure*}

\subsubsection{\ac{siso} Finite-Memory Channels} In particular, we generate each realization of the taps using an indoor hall $5$GHz setting with single-antenna elements. We use the same block length and number of error-correction symbols, as well as the same initial training set $\mySet{D}_0$ as in the synthetic model. This setting may represent a user moving in an indoor setup while switching between different microcells. Succeeding on this scenario requires high adaptivity since there is considerable mismatch between the train and test channels. The test is carried out using a sequence of difference realizations illustrated in Fig.~\ref{fig:COSTChannel}, whereas the initial training still follows the taps illustrated in Fig.~\ref{fig:synthetic_train_channel}. The two main figures, Fig.~\ref{fig:SISOcostBERvsBlock} and Fig.~\ref{fig:SISOcostBERvsSNR} illustrate gains of up to 0.6dB by using our scheme compared to other methods. 

\subsubsection{Memoryless \ac{mimo} Channels} For the current \ac{mimo} setting, we compose the test channels from only $T_p=T_d=40$ blocks and increase the number of users and antennas to $N = K = 8$. To simulate the channel matrix $\myMat{H}$, we follow the above \ac{siso} description and create $8 \times 8 = 64$ \ac{siso} COST 2100 channels; Each simulated channel corresponds to a single entry $\left( \myMat{H}\right)_{n,k}$ with $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$. Moving to results, one may observe the respective graphs Fig.~\ref{fig:costBERvsBlockMIMO} and Fig.~\ref{fig:costBERvsSNRMIMO}, which show an unusual gain of up to 1.5dB approximately, as the joint and online methods are unable to compete with the proposed meta approach.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/costBERvsBlock.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:SISOcostBERvsBlock}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_ber_versus_snr.png}
    \caption{Coded \ac{ber} after 300 blocks vs. SNR.}
    \label{fig:SISOcostBERvsSNR}
    \end{subfigure}
    %
    \caption{\ac{siso} COST 2100 channel, $\Blklen = 136$.}
    \label{fig:SISOCostBER} 
    \figSpace
\end{figure*}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/costBERvsBlock_mimo.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:costBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_ber_versus_snr_mimo.png}
    \caption{Coded \ac{ber} after 40 blocks vs. SNR.}
    \label{fig:costBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} COST 2100 channel, $\Blklen = 96$.}
    \label{fig:CostBERMIMO} 
    \figSpace
\end{figure*}



\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_modular_all.png}
    \caption{Synthetic linear channel, ${\rm SNR} = 11$ dB.}
    \label{fig:synth_modular_online}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_modular_all.png}
    \caption{COST 2100 channel, ${\rm SNR} = 13$ dB.}
    \label{fig:cost_modular_online}
    \end{subfigure}
    %
    \caption{Modular Training - Coded \ac{ber} vs. block index, $\Blklen = 96$.}
    \label{fig:ModularTrainingOnline} 
    \figSpace
\end{figure*}

\subsection{Modular Training Results}
\label{subsec:modular-training}
As discussed before, our approach is best utilized with the model-based architectures. This is due to the model-based structure of the receiver, having fewer parameters than model-free receivers. This fact permits quick adaption with small block size. To further exploit the interpretable structure of the model, we employ a new modular training scheme as explained in Section~\ref{sec:modular-training}. 

We consider a new \ac{mimo} scenario, where only a single user is changing, with the other ones being static. We apply the modular training method: Training the neural networks of a single given user, as described in Subsection~\ref{subsec:DeepSIC}. Fig.~\ref{fig:ModularTrainingOnline} shows the two compared methods, the online-training and online-meta training, executed either with or without the modular training feature (i.e. single user training) for the synthetic linear channel and the COST 2100 channel. We also plot the joint training method for completeness. Observing the plotted curves, one may observe that our modular meta-training achieves superior results compared to the other methods; This validates our two-stage approach. It also strengthens the idea that the knowledge of whichever user is changing may improve the performance of model-based architectures.

\subsection{Pilots Efficiency} 
\label{subsec:pilot-training}
To estimate the efficiency of training with pilots across all methods, we consider a new transmission model, where a pilot block is transmitted before each data block as in Fig.~\ref{fig:pilots_eff_transmission}. The same number of data blocks is transmitted as in Subsection~\ref{subsec:synth_simulation_results} and Subsection~\ref{subsec:cost_simulation_results} for the \ac{mimo} cases, where $T_d = 50$ and $T_d = 40$, respectively. Now, we set the length of data blocks to constant 5000 bits in order to check adaption over long blocks. No coding scheme is employed; Instead, we only train on the pilot blocks, whose size varies. Pilot blocks are immediately inserted into the buffer in the meta-training approach, as specified in Algorithm~\ref{alg:online-meta-learning}.  

Moving to results, we consider the flat \ac{mimo} channels as above. Here, one may observe that our training approach is preferable to  the other approaches at most lengths, for the linear synthetic as well as the COST 2100 channel (Fig.~\ref{fig:pilots_efficiency_mimo}). We highlight that our method is able to better utilize the model-based architecture of the detector to it's maximum efficiency, compared to model-free architecture, exploiting the pilots for better performance and consistently lower error rates than the other compared methods.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.67\textwidth,height=0.09\textheight]{fig/pilots_eff_transmission.png}
    \caption{The new data transmission model with periodic transmission of pilots.}
    \figSpace
    \label{fig:pilots_eff_transmission}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_pilots_efficiency_mimo.png}
    \caption{Synthetic channel, ${\rm SNR} = 12$ dB.}
    \label{fig:synth_pilots_efficiency_mimo}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_pilots_efficiency_mimo.png}
    \caption{COST 2100 channel, ${\rm SNR} = 14$ dB..}
    \label{fig:cost_pilots_efficiency_mimo}
    \end{subfigure}
    %
    \caption{SER vs. pilots size with $\Blklen = 96$.}
    \label{fig:pilots_efficiency_mimo} 
    \figSpace
\end{figure*}


==> sections_v0/system_model.tex <==
\section{System Model}
\label{sec:Model}
\vspace{-0.1cm}

Here, we describe the system model for which the online training algorithm is designed. We begin by presenting the channel model in Subsection~\ref{subsec:Channel}. Thereafter, we formulate the communication protocol and the problem in Subsections~\ref{subsec:Transmission} and \ref{subsec:Problem}, respectively. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth,height=0.1\textheight]{fig/transmission_model.png}
    \caption{Transmission model. The channel is constant within each block and  changes across blocks. }
    \figSpace
    \label{fig:transmission}
\end{figure*}

% \textcolor{red}{This section needs to be re-organized. Before describing the communication protocols, which is divided into blocks, I think we should introduce the block-wise varying channel model. Second, the detection scenario  in Subsec. \ref{subsec:Transmission} does not discuss detection; it explains the considered transmission protocol.  Finally, the formulated problem does not really capture the problem that we are trying to solve.
% \\
% So we should start with the generic channel model, and emphasize that the actual input-output relationship in \eqref{eqn:ChModel1} may be highly complex. We should also indicate that the variations in the channel between blocks are often not arbitrary and can be due to, e.g., movement of some of the communicating entities. We build on this property in two aspects of our solution - the fact that we train on one channel for to following one, and the modular training procedure. \\ 
% Then, we should proceed by describing the communication protocol, where you explain the division into pilots and data, and don't forget to clarify that coding includes both \ac{fec} and error detection - our solution relies on their existence. \\
% Finally, present the formulation of the problem, which should be what we are trying to solve. Now, we are not designing a symbol detection mechanism that imitates the MAP rule, we are proposing an algorithm which allows a \ac{dnn} aided receiver, whose input-output mapping is dictated by a parameter vector $\theta$, to adapt its parameters over time in order to continuously provide low error rates over the data blocks. 
% }

%-----------------------------------
%	Block-Fading Channel Model
%-----------------------------------
\vspace{-0.2cm}
\subsection{Channel Model}
\label{subsec:Channel}
\vspace{-0.1cm} 

We consider communications over casual finite-memory block-wise varying channels with multiple users. The channel output depends on the last $\Mem >0$ transmitted symbols, where $\Mem$ is the memory length. The channel is constant within a block of $\Blklen$ channel uses, which corresponds to the coherence duration of the channel. 

Let $\myVec{S}_{i,j}\in\mySet{S}^K$ be the symbol transmitted from constellation $\mySet{S}$ at the $i$th time instance, $i \in \{1,2,\ldots, \Blklen\}:= \Blkset$, of the $j$th block. Here, the constellation size is $|\mySet{S}|=\CnstSize$ and $K$ denotes the number of symbols transmitted at each time instance, e.g., the number of users transmitting simultaneously in an uplink communications channel.
The channel output is denoted by $\myY_{i,j}\in \mySet{Y}^N$, where $N$ represents the number of receive antennas, and is given by a stochastic function of the last $L$ transmitted symbols 
%$\myVec{S}_{i,j-\Mem+1},\ldots, \myVec{S}_{i,j}$.
$\myState_{i,j} := [\myVec{S}_{i,j-\Mem+1},\ldots, \myVec{S}_{i,j}]^T$.  
Specifically, by defining the $j$th transmitted block as $\myS_j := \{\myVec{S}_{i,j}\}_{i\in \Blkset}$ and its corresponding observations as $\myY_j:= \{\myY_{i,j}\}_{i\in \Blkset}$,  the conditional distribution of the channel output given its input satisfies   
\begin{equation}
	\label{eqn:ChModel1}
	P_{\myY_j | \myS_j}\left(\myVec{y}_j | \myVec{s}_j \right)  = 
	\prod\limits_{i\!=\!1}^{\Blklen}P_{\myY_{i,j} |\myState_{i,j}}\left(\myVec{y}_{i,j} |\mystate_{i,j}\right).  
\end{equation}
In \eqref{eqn:ChModel1}, the lower-case notations $\myVec{y}_{i,j}$ and $\myStateR_{i,j}$ represent the realizations of the \acp{rv} $\myY_{i,j}$ and $\myState_{i,j}$, respectively. We set $\myVec{S}_{i,j} \equiv \myVec{0}$ for $i<0$, i.e., we assume a guard interval of at least $\Mem-1$ time instances between blocks.

%Practical communication scenarios are highly complex; 

The input-output relationship in \eqref{eqn:ChModel1} describes a generic channel model with block-wise temporal variations. These  channel variations, i.e., changes between different values of the block index $j$, can often be attributed to some phenomena, e.g. a  movement  of one or several of the communicating entities. %Our two-stage training method is tailored for these complex scenarios, exploiting domain knowledge, whereas naive algorithms fail. 
We do not impose a specific model on the channel observed in each block, representing it by the generic conditional distribution in \eqref{eqn:ChModel1}, which can take a complex and possibly intractable form. Two important special cases of this channel model include:
\begin{enumerate}
    \item \emph{\ac{siso} Finite-Memory Channels}: The first type of channels considered in this work is the multipath \ac{siso} case; That is, we set $N=K=1$. 
    \item \emph{Flat \ac{mimo} Channels}: Another channel of interest is the memoryless ($L=1$) \ac{mimo} channel, where $N>1$ and $K>1$. Such settings specialize multi-user uplink \ac{mimo} systems, where $K$ is the number of single-antenna transmitters. 
\end{enumerate}




%-----------------------------------
%	Transmission
%-----------------------------------
\vspace{-0.2cm}
\subsection{Communication Protocol}
\label{subsec:Transmission}
\vspace{-0.1cm}  

We consider the scenario illustrated in Fig.~\ref{fig:transmission}, where a total of $T_p$ pilot blocks and $T_d$ data blocks are transmitted sequentially. That is, blocks indexed $j\in\{0,\ldots,T_p-1\}$ are known pilots,  while $j\in\{T_p,\ldots,T_p+T_d-1\}$ are data blocks. The pilots blocks convey a known message, whereas the data blocks are unknown and are utilized to test the proposed schemes. Each data block, i.e., $\myVec{S}_j$ for $j\in\{T_p,\ldots,T_p+T_d-1\}$, is encoded into a total of $B$ symbols using both \ac{fec} coding and error detection codes. Error detection codes, such as cyclic redundancy check, allow the receiver to identify the presence of errors in the decoding procedure.

%-----------------------------------
%	Problem Formulation
%-----------------------------------
\vspace{-0.2cm}
\subsection{Problem Formulation}
\label{subsec:Problem}
\vspace{-0.1cm}  
We consider the problem of symbol detection in the generic channel model formulated in Subsection~\ref{subsec:Channel}. The fact that we do not impose a specific model of the channel, allowing its input-output relationship to take complex forms in each block, combined with the availability of data based on the protocol detailed in Subsection~\ref{subsec:Transmission}, motivate the usage of \ac{dnn}-aided receivers. The core challenge in applying \ac{dnn}-aided receivers for the considered channel model stems from its temporal variations. Our objective is thus to derive a training algorithm that allows \ac{dnn}-aided receivers in recovering the transmitted data from the channel outputs  $\{\myVec{Y}_j\}_{j=T_p}^{T_p+T_d-1}$.

In particular, we let $\Weights$ denote the parameters of the \ac{dnn}-aided receiver, i.e., the weights of the neural network. These parameters dictate the receiver mapping, which, for a given $\Weights$, is denoted by $\hat{\myVec{s}}(\cdot; \Weights):\mySet{Y}^{N\times \Blklen } \mapsto \mySet{S}^{K\times \Blklen}$, i.e., $\hat{\myVec{s}}(\myVec{y}; \Weights)$ denotes the symbol block recovered\footnote{while the \ac{dnn}-aided receiver is formulated here as outputting symbol decisions, one can also adapt the formulation to soft (probabilistic) decisions. } by the receiver parameterized with $\Weights$ when applied to the channel output block $\myVec{y}$. By using the abbreviated terms  $\hat{\myVec{s}}_j(\Weights)$ to denote the symbols detected based on the channel output of the $j$th block, with $\hat{\myVec{s}}_{i,j}(\Weights) \in \mySet{S}^K$ being its $i$th symbol, $i \in \Blkset$, our goal is to propose an algorithm which allows a DNN-aided receiver  to  continuously provide low error rates over the data blocks:
\begin{equation}
\label{eqn:ErrorRate}
	\mathop{\min}\Big(\frac{1}{\Blklen}\sum_{i=1}^{\Blklen} \Pr\left( \hat{\myVec{s}}_{i,j}(\Weights_j) \neq  \myVec{S}_{i,j} \right)\Big), \qquad j\in\{T_p,\ldots,T_p+T_d-1\}. 
\end{equation}
The parameter vector $\Weights$ in \eqref{eqn:ErrorRate} is allowed to change between blocks, namely, the \ac{dnn}-aided receiver can adapt its parameters over time. As our problem formulation does not impose a specific structure on the \ac{dnn}-aided receiver, we first consider an online adaptation mechanism which is invariant of the structure of the \ac{dnn}-aided receiver, after which we show how one can further benefit when the \ac{dnn} is of an interpretable modular architecture.

==> sections_v1/abstract.tex <==
\begin{abstract} 
Many emerging digital communication applications \SangwooCmt{are required} to operate in dynamic and complex environments. Recent years have witnessed a growing interest in the application of deep neural networks (DNNs) for receiver design, which can potentially operate in complex environments without relying on knowledge of \SangwooCmt{the} channel model and its parameters. However, the dynamic nature of communication channels often leads to rapid distribution shifts. In order to track temporal variations, DNN-based receivers may be required to periodically retrain %in an efficient manner 
without inducing substantial overhead. 
%	
This paper formulates a data-efficient two-stage training method that facilitates rapid online adaptation. Our training mechanism uses a predictive meta-learning scheme to learn to train rapidly from both local and global variations\SangwooCmt{, which is applicable to any generic DNN-based receivers and requires no transmission of new pilot data for training}. Moreover, we leverage on the explainable structure of model-based DNN-aided symbol detectors, training only specific sub-blocks of the model. The latter, referred to as modular training, is combined with predictive meta-learning  to assist in the quick adaptation of the receiver to rapidly-varying channels \SangwooCmt{when using model-based deep symbol detectors.} 
Our extensive numerical evaluations \SangwooCmt{include a synthetic linear channel, a synthetic non-linear channel and a COST 2100 channel.} Our results demonstrate that the \SangwooCmt{proposed online training} scheme allows receivers to  outperform previous  approaches \SangwooCmt{by a margin of up to 2.5dB in coded bit error rate over rapidly-varying scenarios.}
\end{abstract}

==> sections_v1/conclusion.tex <==
\section{Conclusion}
	\label{sec:Conclusions}
	\vspace{-0.1cm}
We proposed an online meta-learning algorithm for training data-driven receivers. Our approach aids the the receiver in tracking channel variations, incorporating both short-term and long-term relations. We combine three key ingredients that enable the tracking of rapidly time-varying channels: a model-based \ac{dnn} architecture; an online adaptation scheme with optimized initial weights; and the use of coded blocks for self-supervised training\SangwooCmt{, which requires no transmission of new pilots blocks}. Furthermore, We introduced a modular training scheme,  that exploits the interpretable structure of model-based detectors to aid in quick adaptation to rapidly-varying channels. Numerical study demonstrates that, by properly integrating these methods, model-based receivers trained with the meta-training algorithm and modular training  outperform joint and online training approaches and are better able to track changing channels.

==> sections_v1/introduction.tex <==
\section{Introduction}
\vspace{-0.1cm} 
	
% Paragraph - need to operate in complex channel conditions
Traditional receiver design is dominated by methods that are based on statistical models. Such conventional receivers rely on  mathematical models that describe the transmission process, signal propagation, interference, and many other components of the system that affect end-to-end communications. These statistical models typically adopt simplifying assumptions 
that make them tractable and understandable, and use parameters that vary over time as the channel conditions change.   The need for an accurate and simplified model may constitute a notable limitation in future communication technologies.  As high frequency bands and spectrum sharing  become widespread, current simplified models used for the channel, interference, and noise may be inaccurate \cite{xia2020mimo}. Moreover, emerging antenna architectures result in complex modelling of the transmission and reception process \cite{shlezinger2020dynamic}, while the deployment of intelligent surfaces notably complicates channel estimation \cite{alexandropoulos2021hybrid}. Furthermore, signalling in high frequencies is often prone to hardware non-idealities affecting the overall model, either unintentional or due to using limited hardware, e.g., few-bit \acp{adc} \cite{shlezinger2018asymptotic} and non-linear amplifiers \cite{singya17PA}.  This makes conventional channel-model-based techniques significantly more complex.
	
% Paragraph - deep learning for receivers
An alternative data-driven approach is based on deep learning. 
Deep learning systems have demonstrated unprecedented success in various applications, ranging from computer vision to natural language processing, and recently also digital communications and receiver design \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, oshea2017introduction}. While traditional receiver algorithms are channel-model-based, %relying on mathematical modeling of the signal transmission, propagation, and reception, 
\acp{dnn} are model-agnostic, and are trained from data. \ac{dnn}-aided receivers can operate efficiently in scenarios where the  channel model is unknown, highly complex, or difficult to optimize for~\cite{farsad2018neural}.

% Paragraph - inherent challenge due to temporal variations
Despite their potential in implementing digital receivers \cite{shlezinger2020inference,farsad2020data}, deep learning solutions are subject to several challenges that limit their applicability in important communication scenarios. A fundamental difference between digital communications and traditional deep learning applications stems from the dynamic nature of communication systems, and particularly of wireless channels.  \acp{dnn} consist of highly-parameterized models that can represent a broad range of mappings. As such, massive data	sets are typically required to learn a desirable mapping.  The dynamic nature of communication channels implies that the statistical model can change considerably over time, and thus a \ac{dnn} trained for a given channel may no longer perform well on future channel realizations. %\ac{dnn}-aided receivers are thus likely to require frequent retraining, at the cost of degraded spectral efficiency due to pilot transmissions. % which adds to the increased computational burden involved in training \acp{dnn}.

To apply \ac{dnn}-aided transceivers in time-varying channels, two main approaches are considered in the literature. The first  attempts to learn a single mapping that is applicable to a broad range of channel conditions. This class of methods includes the straightforward approach of training a \ac{dnn} using data corresponding to an extensive set of expected channel conditions, which is referred to as {\em joint learning}\cite{oshea2017introduction, xia2020note}. An additional related method trains in advance a different network for each expected channel, and combines them as a deep ensemble \cite{raviv2020data}. However, these strategies typically require a large amount of training data, and  deviating from the training setup, i.e., operating in a channel whose characteristics differ from those observed during training, can greatly impair performance \cite{park2020learning}. 

An alternative strategy is to track the channel variations. This can be achieved by providing the \ac{dnn} with a model-based channel estimate \cite{he2020model,honkala2021deeprx,khani2020adaptive, samuel2019learning, goutay2021machine}. However,  channel estimation involves imposing a relatively simple model on the channel, e.g. a linear Gaussian model, which may be inaccurate in some setups. 
When operating without channel knowledge, tracking the channel involves periodically retraining the network. To provide data for retraining, one must either transmit frequent pilots, or, alternatively, use decoded data for training. Such self-supervised training can be implemented by either using successfully decoded \ac{fec} codewords, as  in \cite{shlezinger2019viterbinet, teng2020syndrome}, or  by providing a measure of confidence per each symbol and selecting those with the highest confidence for retraining, as proposed in \cite{sun2020generative}. Nonetheless,  the volumes of data one can obtain in real-time, either from pilots or from decoded transmissions, are limited and are not at the scale of typical data sets used for training \acp{dnn}. Retrained \ac{dnn}-aided receivers should thus utilize compact \ac{dnn} architectures. This can be achieved without compromising accuracy by using hybrid model-based/data-driven receivers that incorporate domain knowledge. Following this principle, data-driven implementations of the Viterbi scheme \cite{viterbi1967error},  BCJR method \cite{bahl1974optimal}, and  iterative \ac{sic}  \cite{choi2000iterative} were proposed in \cite{shlezinger2019viterbinet,shlezinger2020data, shlezinger2019deepSIC}, respectively. Yet, even with compact architectures, relatively large data sets are still required and typical \ac{dnn} training procedures are likely to induce non-negligible delay. 

The ability to retrain quickly is highly dependent on the selection of a suitable initialization of the iterative training algorithm. While the common strategy is to use random weights, the work \cite{shlezinger2019viterbinet} used the previous learned weights as an initial point for  retraining. 
An alternative approach is to optimize the initial point via meta-learning \cite{park2020meta,simeone2020learning,jiang2019mind,park2020learning}. Following this approach, one not only retrains, but also optimizes the hyperparameters that dictate the retraining process. In particular, it was shown in \cite{park2020learning} that by optimizing the initial weights, rather than using random weights or the previous ones, the receiver can quickly adapt to varying channel conditions. 
%Furthermore, to enable online training in a self-supervised manner, it was proposed in \cite{shlezinger2019viterbinet} to exploit the presence of \ac{fec} codes, commonly utilized in digital communications, to retrain in a decision-directed fashion.


In this work we propose an online training algorithm to enable rapid adaptation of channel-model-agnostic \ac{dnn}-aided receivers from scarce pilots. Our algorithm considers both long and short term variations in the channel: We choose the initial weights by a communication-adapted meta-learning algorithm \cite{finn2017model}, which we enhance to facilitate training for future (predicted) channel realizations, while tracking local variations in a self-supervised manner. The latter is achieved by exploiting the presence of \ac{fec} codes, commonly utilized in digital communications, to retrain in a decision-directed  fashion as in \cite{shlezinger2019viterbinet,teng2020syndrome}.


Moreover, with suggest to adapt this meta-learning scheme to model-based deep receivers. Model-based deep learning refers to a family of techniques for designing systems which combine principled model-based algorithms with data-driven deep learning techniques \cite{shlezinger2020model}. Hybrid design techniques, such as deep unfolding \cite{monga2021algorithm}, neural augmentation \cite{satorras2020neural}, and \ac{dnn}-aided algorithms \cite{farsad2021data}, gave rise to a multitude of deep receiver architectures, including, e.g., \cite{shlezinger2020data,samuel2019learning,he2020model,nachmani2018deep,balatsoukas2019deep, be2019active,shlezinger2019deepSIC, shlezinger2019viterbinet}. These hybrid  model-based/data-driven receivers build on existing communication models and incorporate deep learning into their design, rather than replace the known model altogether. These receivers can be agnostic to the channel-model, imitating the operation of a suitable detection algorithm without relying on knowledge of the actual channel model and its parameters. Moreover, they are much more compact in terms of parameters, thus are faster to train and require fewer training samples to reach convergence \cite{shlezinger2020model}.
We propose to exploit the the explainable structure of model-based deep receivers in order to re-train only specific modules of the architecture. This new approach to online training, referred to as \textit{modular training}, enables adaptation in quickly-changing scenarios as one has fewer parameters to train. 

% to train This enabling the use of self-generated labels that extend the availability of supervised data beyond the pilot blocks. 
Our main contributions are summarized as follows:
\begin{itemize}
    \item \textbf{Predictive online meta-learning algorithm:} We tailor \ac{maml} \cite{finn2017model} to the prediction of time-varying channels. The proposed method is designed to ensure that a small number of gradient updates, calculated by training on the last decoded block, minimizes the loss (or error) on the next data block. \SangwooCmt{The method developed is generic, and applicable to any \ac{dnn}-aided receiver.}
    \item \textbf{Modular training of interpretable architectures:} 
    \SangwooCmt{We next focus on hybrid model-based/data-driven receivers that leverage the structure of multipath channels.} \SangwooCmt{We} propose to \SangwooCmt{only retrain} specific modules of the receiver architecture \SangwooCmt{that need adaptation due to} temporal variations of the channel. \SangwooCmt{Fast and efficient adaptation of the machine learning modules utilize a variant of MAML referred to as almost-no-inner-loop  (ANIL) \cite{raghu2019rapid}, that incorporates \emph{a priori} information about variability of the channels.}
    
    
    \item \textbf{Extensive Experimentation:} We extensively evaluate the proposed training scheme for both \ac{siso} and \ac{mimo} systems, considering three different time-varying channel profiles: linear synthetic channel, a non-linear synthetic channel, and a COST 2100 \cite{liu2012cost}  channel.
    We show gains of up to 1.5 dB in coded \ac{ber}, compared to joint and online approaches, over a set of challenging channels. \SangwooCmt{Compared to state of the art, we show that the proposed schemes offer advantages in terms of average \ac{ser} over rapidly changing scenarios, while reducing the pilot overhead.}
\end{itemize}

 The rest of this paper is organized as follows:  Section~\ref{sec:Model} details the system model, while Section~\ref{sec:Hybrid Meta-Learning for Data-Driven Receivers} presents the meta-learning algorithm. In Section~\ref{sec:modular-training} we focus on model-based deep receivers and show how to exploit their interpretable structure via modular training. Finally, experimental results and concluding remarks are detailed in Section~\ref{sec:Simulation} and Section~\ref{sec:Conclusions}, respectively.

Throughout the paper, we use boldface letters for vectors, e.g., ${\myVec{x}}$; $({\myVec{x}})_i$ denotes
the $i$th element of ${\myVec{x}}$. %We use upper-case letters for \acp{rv}, and lower-case letters for deterministic quantities. 
Calligraphic letters, such as $\mySet{X}$, are used for sets, 
and $\mySet{R}$ is the set of real numbers.



==> sections_v1/method.tex <==
\section{Predictive Online Meta-Learning for DNN-Aided Receivers}
	\label{sec:Hybrid Meta-Learning for Data-Driven Receivers}
	\vspace{-0.1cm}
	In this section we study parameter adaptation of a generic \ac{dnn}-aided receiver to continuously maintain low error rates in time-varying channels. Modification of these weights involves training, which requires the receiver to obtain recent examples of pairs of transmitted blocks and corresponding observed channel outputs. This gives rise to two core challenges. First, while one can use pilots, the time-varying nature of the channel implies that  pilot-based examples are likely to not represent the  channel conditions for some or all of the data blocks. In addition, even if one can extract labeled training data from blocks containing information messages, when the channel varies quickly, the amount of data from the instantaneous channel may be limited. % Combining this with the typical lengthy duration of \ac{dnn} training procedures makes online adaptation of \ac{dnn}-aided receivers a challenging task. 
	
	These challenges are tackled by the proposed online meta-training algorithm. To describe this algorithm, we begin by introducing self-supervised training in Subsection~\ref{subsec:Online} for slow-fading channels, and then we extend online training to rapidly time-varying channels. The resulting algorithm is detailed in Subsection~\ref{subsec:MetaLearningDiscussion}.

%-----------------------------------
%	Decision-Directed Online Training
%-----------------------------------
\vspace{-0.2cm}
\subsection{Self-Supervised Online Training}
\label{subsec:Online}
\vspace{-0.1cm} 

% \textcolor{red}{At this point in the paper we have already formulated the channel model and the problem. So now we need to gradually lead towards our solution based on the model. So I recommend starting the section by:\\
% Start by explaining that since we consider the operation of \ac{dnn}-aided receivers in complex channels, as detailed in Subsection~\ref{subsec:Channel}, one would need to periodically re-train the \ac{dnn} in order to preserve reliable operation in time-varying conditions. \\
% Then, explain that the core algorithmic challenge in doing so stems from the availability of data. Training requires data corresponding to the instantaneous channel conditions being observed currently, while the generic protocol detailed in Subsection-??? implies that pilots, which can be used to formulate a labeled training set, are scarce and may not correspond to the current channel. }

% We regard the problem of \ac{dnn}-aided receivers in complex time-varying channels, as detailed in Subsection~\ref{subsec:Channel}, where the distribution of the channel output $\myY$ changes with time. As the deviation between the trained-on channel and the tested one increases, one obviously needs to periodically re-train the receiver to preserve high performance operation. 

The first part of our online adaptation mechanism is based on self-supervision, which extracts training data from information-bearing blocks. The approach follows \cite{shlezinger2019viterbinet} by re-using confident decisions via the re-encoding of a successfully decoded word for use in online training. 
%
%Following this approach, the parameters of a \ac{dnn}-aided receiver are adapted on a block by block basis; That is, on any incoming block $\myVec{y}_j$. Even if the deep symbol detector is not trained for the instantaneous channel realization from which $\myVec{y}_j$ is generated and thus its estimate $\hat{\myVec{s}}_j$ may differ from the true transmitted symbol vector, the \ac{fec} decoder can still correct these errors, as long as they are within the Hamming distance of the code. Specifically, the channel decoder takes as input the estimated block $\hat{\myVec{s}}_j$, and outputs a decoded message along with the number of errors, as an indication of the correctness of its decoded message. When decoding is correct, i.e. the number of errors is 0, the decoded and demodulated message $\hat{\myVec{m}}_j$ is encoded and modulated into the estimated transmitted symbols  $\myVec{s}_j$.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/self-supervised online training figure.png}
    \vspace{-0.6cm}
    \caption{Self-supervised online training based on channel coding.}
    \label{fig:self-supervised training}
\end{figure}
	

% \textcolor{red}{We can consider adding a figure visualizing how online training operates. It can be divided into two parts - symbol detection and online training. }

% Specifically, the detector for the $j$th block is parameterized by the weight vector $\Weights_j$, which is applied to $\myVec{y}_j$. When decoding is successful, one can confidently generate a 

\SangwooCmt{First, we initialize the parameter vector $\Weights_{T_p}$ by training over the obtained $T_p$ pilot blocks.} Then, for each information block \SangwooCmt{$j\in\{T_p,\ldots,T_p+T_d-1\}$}, when decoding is reported by the decoder to be correct, the re-encoded data pair $\{\myVec{s}_{j}, \myVec{y}_{j}\}$ is used as training data to update the parameters for the next block, i.e., to generate $\Weights_{j+1}$. \SangwooCmt{The same training is applied to the receiver during pilots and information blocks transmission.} Since symbol detection can be treated a classification task, this is achieved by minimizing the empirical cross entropy loss as
\begin{align}
\label{eq:meta_1}
  \mathop{\arg \min}_{\Weights} \left\{ \mySet{L}_{j}(\Weights) = -\sum_{i=1}^{\Blklen}\log \hat{P}_{\Weights}\left(\myVec{y}_{i,j}|\myStateR_{i,j} \right)\right\}.
\end{align}
In (\ref{eq:meta_1}), the  probability $\hat{P}_{\Weights}\left( \myVec{y}  |  \myStateR\right)$ is the soft output of the \ac{dnn}-aided receiver corresponding to $\myStateR$ when applied to the data block $ \myVec{y}$. The optimization problem in \eqref{eq:meta_1} is approximately solved using gradient-based optimization with some learning rate $\eta$, i.e., via $I$ iterations of the form
 \begin{align}
\label{eq:local_update} % \label{eq:meta_1}
\Weights_{j+1}^{(t+1)} = \Weights_{j+1}^{(t)} - \eta \nabla_{\Weights_{j+1}^{(t)}}\mySet{L}_{j}(\Weights_{j+1}^{(t)}).
 \end{align}
 %where $\eta > 0$ is the learning rate. 
 
 The computation of the gradient steps requires an initialization $\Weights_{j+1}^{(0)}$, which is a hyperparameter of the training procedure. We henceforth denote this hyperparameter vector used for self-supervised training of $\Weights_{j+1}$ as  $\HyperParams_{j+1}$, i.e., $\Weights_{j+1}^{(0)} = \HyperParams_{j+1}$. 
 The gradient in \eqref{eq:local_update} is typically approximated via random sampling among available $B$ symbols within the block to implement \ac{sgd} and its variants, typically used for training DNNs \cite[Ch. 4]{goodfellow2016deep}.  The online training scheme is presented in Fig.~\ref{fig:self-supervised training}.
%
%In order to enable an adaptation mechanism, the receiver maintains at each block index $j$ a vector of hyperparameters $\HyperParams_j$. %\NirCmt{Do we need to introduce the data buffer at this stage? We do not really use it here, but for meta-learning. So I guess the main question is whether the purpose of this section is to discuss how online self-supervised training is done in the literature, or to explain how we do it here? If we go with the latter, we need to explain that the proposed scheme only observes short-term variations, i.e., those between the current block and the next one, and thus missing out on long-term variation, such as patterns of variations observed in the past. To be able to also account for these longer variations, we save decisions in the buffer, whose usage is revealed in ths sequel.}.
%
%At each data block $j$, given the initialization hyperparameter vector\NirCmt{Perhaps we should not state here how the initial hyperparameters vector is set, just say that we use some initialization $\HyperParams_j$. Then, when we conclude the section say that the approach used in \cite{shlezinger2019viterbinet} used $\HyperParams_j=\Weights_{j-1}$, which implies that only short-term variations are accounted for in the training procedure, as both the data and the optimization hyperparameters correspond to the current instantaneous channel realization.} $\HyperParams_j$ and successfully decoded blocks' pair $\{\myVec{s}_{j-1}, \myVec{y}_{j-1}\}$, the algorithm updates the model parameters vector $\Weights_j$. 
 %
 For reliable operation, the self-supervision training algorithm exploits the fact that dynamic channels are of continuous nature, and thus one can reasonably assume that the data from the channel observed in the $j$th block is still applicable to the $j+1$th channel realization. Following this line of reasoning,  \cite{shlezinger2019viterbinet} used $\HyperParams_{j+1}=\Weights_{j}$ 
 
 %two main characteristics of digital communications over time-varying channels: 
  %\begin{enumerate}
    %\item The first is the presence of \ac{fec} coding that provides a safe margin and allowing one to recover the transmitted symbols even as a small number of errors occur. The exact number is dependent on the Hamming distance of the \ac{fec} code. Moreover, one can identify when re-encoding is possible, employing the re-encoded block for training. 
    
    %\item The second property exploited is the fact that dynamic channels are of continuous nature; Thus one can reasonably assume that the data from the channel observed in the $j$th time index is still applicable to the $j+1$th channel realization. Following this line of reasoning, the researchers in  \cite{shlezinger2019viterbinet} used $\HyperParams_{j+1}=\Weights_{j}$. 
 %\end{enumerate}
 
In this paper, we contend that this assumption is inadequate for tracking fast-varying channels and should be revised. Adapting locally in a self-supervised manner by setting the hyperparameter $\HyperParams_{j+1}=\Weights_{j}$ accounts for only short term variations, as both the data and the optimization hyperparameters correspond to the current instantaneous channel realization. In order to train effectively from short blocks in complex channels, we propose to incorporate long term relations by altering the setting of the hyperparameter $\HyperParams_{j+1}$ via meta-learning.
 
 %mini-batch. Note  \eqref{eq:local_update} describes a single \ac{sgd} iteration,  multiple iterations are similarly accommodated.

% \textcolor{red}{I recommend concluding the above paragraph by clarifying that the ability to carry out such self-supervision relies on two characteristics of digital communications over time-varying channels: The first is the presence of coding, which allows one to recover re-form the transmitted symbols even when detection has errors as long as these errors are below the Hamming distance of the \ac{fec} code, as well as identify when such re-encoding is possible due to error detection codes. The second property exploited is the fact that dynamic channels are not arbitrarily time-varying, and thus one can train using data corresponding the channel observed during the $j$th while still being applicable in the $j+1$th channel realization. \\
% After saying that, please explain why is this not enough on its own. This will lead us to the need optimize the hyperparameters $\theta_j$ in order to effective online training from short blocks and with few epochs, which is discussed in the following section. This way you lead your readers through your method (which on its own is quite complicated, thus requires a gradual gentle well-motivated introduction of its components). }


%-----------------------------------
%	High-Level Description
%-----------------------------------
\vspace{-0.2cm}
\subsection{Predictive Online Meta-Learning} 
\label{subsec:high-level}
\vspace{-0.1cm}
While online training as described in the previous subsection is successful when the channel variations are relatively slow, i.e., when the block size $\Blklen$ is large enough to allow the aggregation of sufficient self-supervised data, it may fail to track fast changing channels. To tackle this problem, we propose to exploit long-term memory based on previously observed channel variation patterns using meta-learning to optimize the hyperparameter $\HyperParams_{j}$.

%, in contrast to the self-supervised learning which exploits short-term memory. Meta-learning, often referred to as {\em 'learning to learn'} \cite{lemke2015metalearning}, focuses on optimizing the hyperparamters, i.e., parameters which dictate the learning algorithm, rather than being learned by it. In conventional non-meta-learned systems, these hyperparamters, also referred to as inductive bias, are handcrafted by human designers, typically based on abstract guidelines and experience. Meta-learning enables the learning of these parameters  without relying on heuristics.

	
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/FlowChart3.png}
    \caption{Illustration of the operation of the proposed meta-training algorithm \SangwooCmt{in the test phase}.}
    \label{fig:FlowChart1}
\end{figure}

%This allows us to account for the predictive nature of self-supervised online training, where data from the current block is used to train for the subsequent (predicted) channel realization. Incorporating patterns in the channel variations, observed in past blocks, into the predictive detection aids to minimize the overall \ac{ber}.

% \textcolor{red}{Conclude this section by revealing the rationale of our approach to the readers (before digging into the details. This includes two important aspects of our algorithm: \\
% First, that instead of directly applying conventional \ac{maml}, as done in \cite{park2020learning}, we modify its operation to account for the predictive nature of self-supervised online training, where data from the current block is used to train for the subsequent (predicted) channel realization.   \\
% Second, that we use long-term variations in the channel to determine an initialization for the training algorithms which is expected to facilitate rapid training based on channel variation patters between subsequent blocks observed in the past.} 
	

To this end, following the  \ac{maml} framework \cite{finn2017model}, we define the support task as the {\em detection of the current block}; while the query task, for which the parameters should adapt, is the {\em detection of the next block}. 
Upon the reception of a block of channel outputs $\myVec{y}_j$, the method operates in three stages, illustrated as a block diagram in Fig.~\ref{fig:FlowChart1}:
\begin{enumerate}
    \item \emph{Detection}: Each incoming data block $\myVec{y}_j$ is mapped into an estimated symbol block $\hat{\myVec{s}}_j$, with the mapping determined by the current parameters vector $\Weights_{j}$. Then, it is decoded by using an \ac{fec} decoder to produce the demodulated and decoded message $\hat{\myVec{u}}_j$. When decoding is correct, as determined by error detection, the message $\hat{\myVec{u}}_j$ is re-encoded and modulated, producing an estimated transmitted vector $\tilde{\myVec{s}}_j$ (see Section~\ref{subsec:Online}). This block is inserted along with its observations $\myVec{y}_j$ into a labelled buffer $\mathcal{D}_{j}$.  This buffer contains pairs of previously received blocks $\myVec{y}_j$ along with their corresponding transmitted signal $\myVec{s}_j$, or an estimated version thereof. The buffer $\mathcal{D}_j$ contains $D$ such pairs, and is managed in a first-in-first-out mode. A pilot block $(\myVec{s}_j, \myVec{y}_j)$ is directly inserted into  $\mathcal{D}_{j}$ upon reception.
    \item \emph{Online training}: In each data block $j$, if decoding is successful, the weights $\Weights_{j+1}$ are updated by using the hyperparameters $\HyperParams_{j+1}$ and the newly decoded block $(\myVec{s}_{j}, \myVec{y}_{j})$, as detailed in Subsection~\ref{subsec:Online}. Otherwise, no update is carried out. A similar update takes place for pilot block $j$ with pilot block $(\myVec{s}_j, \myVec{y}_j)$.
    \item \emph{Meta-learning}: The hyperparameter {$\HyperParams_{j+1}$} is optimized  to enable fast and efficient adaptation of the model parameter $\Weights_{j+1}$ based on the last successfully decoded block $(\myVec{s}_{j}, {\myVec{y}}_{j})$ using \eqref{eq:local_update}. Adopting MAML \cite{finn2017model}, we leverage the data in the buffer $\mathcal{D}_j$ by considering the problem
    %\NirCmt{I think that the indexing in \eqref{eq:meta_2} is confusing and inconsistent. I think it should be $ \HyperParams_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}(\Weights =  \HyperParams  -  \kappa \nabla_{\HyperParams}\mySet{L}_{j'}(\HyperParams))$. Can you please double check?}:
    %
\begin{align}
    \label{eq:meta_2}
      \HyperParams_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}(\Weights =  \HyperParams  -  \kappa \nabla_{\HyperParams }\mySet{L}_{j'}(\HyperParams)),
\end{align}
% %
% \begin{align}
%     \label{eq:meta_2}
%       \HyperParams_{j +1}  =  \mathop{\arg \min}_{\HyperParams}     \sum_{\{\myVec{s}_{j+1}, {\myVec{y}}_{j +1}\} \in \mathcal{D}_j}     \mySet{L}_{j +1}(\Weights_{j+1} =  \HyperParams  -  \kappa \nabla_{\HyperParams}\mySet{L}_{j}(\HyperParams)),
% \end{align}
where $\kappa >0$ is the meta-learning rate. The parameters $\Weights$ in \eqref{eq:meta_2} follow the same update rule in \eqref{eq:local_update} by using the last available block $(\myVec{s}_{j'}, \myVec{y}_{j'})$ in the buffer  prior to index $j'+1$. Furthermore, in line with \eqref{eq:meta_1}, the loss $\mySet{L}_{j'+1}(\Weights)$ is computed based on data from the {\em following} available block $(\myVec{s}_{j'+1}, \myVec{y}_{j'+1})$. When the buffer $\mathcal{D}_j$ contains a sufficiently diverse set of pairs of subsequent past channel realizations, the hyperparameter obtained via \eqref{eq:meta_2} should facilitate fast training for future channels via \eqref{eq:local_update} \cite{park2020end}. 
\end{enumerate} 

The online-meta training is applied periodically, i.e., once every $F$ blocks. Moreover, if $\Weights_j$ and/or $\HyperParams_j$ are not updated in a given block index $j$, they are preserved for the next block by setting  $\Weights_{j+1} = \Weights_j$ and/or $\HyperParams_{j+1}=\HyperParams_j$.
%
The online adaptation framework %is detailed in the sequel, and 
is summarized in Algorithm~\ref{alg:online-meta-learning}.


\begin{algorithm} %!
\DontPrintSemicolon
\caption{Online Adaptation on Incoming Block $j$}
\label{alg:online-meta-learning}
\KwIn{Step sizes $\eta, \kappa$; number of iterations $I$; threshold $\epsilon$; buffer $\mathcal{D}_{j}$; hyperparameter $\HyperParams_{j}$}
\KwOut{Hyperparameter $\HyperParams_{j+1}$; weights $\Weights_{j+1}$; buffer $\mathcal{D}_{j+1}$}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
%{\bf Initialization} inductive bias $\HyperParams_1$ and ViterbiNet $\Weights_1$ \\
%{\bf Initialization} buffer $\mathcal{D}_1$ as empty, i.e., $\mathcal{D}_1 \leftarrow [ \hspace{0.2cm} ]$ \\
%\For{$j = 1,2,\ldots$}{
Receive ${\myVec{y}}_j$ 	\tcp*{received channel output}
\uIf{Pilot}{
$\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ \tcp*{known pilots} 
  }
  \uElse{
  Equalize and decode ${\myVec{y}}_j$ into  $\hat{\myVec{u}}_j$ \tcp*{data}
  \uIf{Decoding is correct}{
  Modulate  $\hat{\myVec{u}}_j\mapsto\myVec{s}_j$ \; 
$\mathcal{D}_{j} \leftarrow \mathcal{D}_j \bigcup\{(\myVec{s}_j, {\myVec{y}}_j)\}$ 
  }
%   \uElse{pass
%   }
  }
\nonl\texttt{Online predictive meta-learning (every $F$ blocks)}\;
Set $\HyperParams_{j+1}^{(0)} = \HyperParams_j$\; \label{stp:onlineStart}
\For{$i=0,1,\ldots$}{
\label{stp:Random} Randomly select block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})\in \mathcal{D}_{j}$\; % except for the last block in the buffer $\mathcal{D}_j$\\  
      {\uIf{$(\myVec{s}_{j'}, {\myVec{y}}_{j'})\notin \mathcal{D}_{j}$}{
% pass;  
%   }
%   \uElse{
  go back to line \ref{stp:Random} \tcp*{invalid data for meta-learning}
  }
  }
  Set $\hat{\HyperParams}^{(0)} = \HyperParams_{j+1}^{(i)}$\;
    \For{$t=0,1,\ldots,I-1$}{
   Use block $(\myVec{s}_{j'}, {\myVec{y}}_{j'})$ to compute \tcp*{support task}
      \begin{equation*}
\hat{\Weights} = \hat{\HyperParams}^{(t)} -\eta\nabla_{\hat{\HyperParams}^{(t)}} \mySet{L}_{j'}(\Weights=\hat{\HyperParams}^{(t)}). \end{equation*} \;
    Use subsequent block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})$ to update \tcp*{query task}
  \begin{equation*}
\hat{\HyperParams}^{(t+1)} = \hat{\HyperParams}^{(t)} - \kappa \nabla_{\hat{\HyperParams}^{(t)}}\mySet{L}_{j'+1}(\Weights =\hat{\Weights}). 
\end{equation*}
    }
    Update hyperparameter as $\HyperParams_{j+1}^{(i+1)} =\hat{\HyperParams}^{(I)}$ \tcp*{meta-update}
% Update the parameters with $I$ iterations on the selected block $(\myVec{s}_{j'}, {\myVec{y}}_{j'})$ via \eqref{eq:local_update} as %\tcp*{local update}
%   \begin{equation*}
% \hat{\Weights}_{j+1} = \HyperParams_{j+1}^{(i)}-\eta\nabla_{\HyperParams_{j+1}^{(i)}} \mySet{L}_{j}(\HyperParams_{j+1}^{(i)}). \end{equation*} \;
% Evaluate loss at block $j+1$% $\hat{\Weights}_{j+1}$ for block $j+1$ computed as
% , $\mySet{L}_{j+1}(\hat{\Weights}_{j+1})$\;
% Update hyperparameter $\HyperParams_{j+1}$ via \tcp*{meta-update}
%   \begin{equation*}
% \HyperParams_{j+1}^{(i+1)} = \HyperParams_{j+1}^{(i)} - \kappa \nabla_{\HyperParams_{j+1}^{(i)}}\mySet{L}_{j+1}(\hat{\Weights}_{j+1}). 
% \end{equation*}
}
Set hyperparameter $\HyperParams_{j+1} =\HyperParams_{j+1}^{(i+1)}$ \;
\nonl\texttt{Online learning (on each block)} \;
{\uIf{(Pilot) or (Decoding is correct)}{

 Train $\Weights_{j+1}$ with $({\myVec{s}}_j, {\myVec{y}}_j)$ and initialization $\HyperParams_{j+1}$  via \eqref{eq:meta_1} \tcp*{update} 
  }
  \uElse{ 
      $\Weights_{j+1} \leftarrow \Weights_j$ \tcp*{no update}
  }
  $\mathcal{D}_{j+1}\leftarrow \mathcal{D}_{j}$ \label{stp:onlineEnd} \tcp*{keep buffer}
  }
 %}
\end{algorithm}

% TODO NIR CONTINUE FROM HERE 13-Dec
%-----------------------------------
%	Discussion
%-----------------------------------
\vspace{-0.2cm}
\subsection{Discussion} 
\label{subsec:MetaLearningDiscussion}
\vspace{-0.1cm}
Algorithm~\ref{alg:online-meta-learning} is designed to enable rapid online training from scarce pilots by simultaneously accounting for short-term variations, via online training, and long-term variations, using the proposed predictive meta-learning. \SangwooCmt{The proposed method does not require the transmission of additional pilots during the test phase. Rather,  data is generated in a self-supervised way, employing the current \ac{dnn}-aided receiver and \ac{fec} codes, similar to the online training scheme in \cite{shlezinger2019viterbinet}. This self-training mechanism adapts the \ac{dnn}-aided receiver as the channel changes during test phase. The method is designed for scenarios where the channel changes continuously; If the channel remains constant or changes only slightly, one should be adapting $\Weights$ only during training phase.} 

Compared to joint learning, which uses many channel realizations to train the parameters $\Weights$, we adapt the hyperparameter, i.e., the initial weights for the \ac{sgd} updates, based on actual realization observed after deployment. This builds upon the insight that, while past realizations are likely to differ from the current channel and thus may not contribute to training the \ac{dnn}, they can provide an accurate representation of how the channel varies between blocks. This may improve over online training \cite{shlezinger2019viterbinet}, which assumes the subsequent channel to bear similarity to the current one, without accounting for temporal variation patterns observed in the past. 

The gain associated with  Algorithm~\ref{alg:online-meta-learning} comes at the cost of additional complexity. The additional complexity can be controlled by modifying the number of meta-learning iterations $I$ and/or changing the meta-learning frequency $F$. One can also consider gradually adjusting these key parameters over time, balancing the excessive computational burden based on the current load, mobility level, and power conditions. Furthermore, the rapid growth and expected proliferation of dedicated hardware accelerators for deep learning applications \cite{chen2019deep} indicates that the  number of hardware-capable digital communication devices will increase. Such devices are expected to be able to carry out the needed computations associated with online meta-learning in real-time.

The usage of meta-learning techniques to facilitate \ac{dnn}-aided communications in time varying channels was also considered in the recent literature in \cite{yuan2020transfer,zhang2021embedding, wang2021jointly, jung2021meta}, with applications for deep receivers  studied in \cite{park2020learning, cohen2021learning}. 
%Considering related works, paper \cite{park2020learning} focuses on an IoT scenario, where a meta-learning scheme is devised to aid a black-box demodulator in quick adaptation to new end-to-end channel conditions from few pilots. 
Though sharing the meta-learning concept, our proposed algorithm fundamentally differs from these previous works is several core aspects. First, references \cite{park2020learning,cohen2021learning} assumed the availability of a relatively large number of pilots per coherence block, which is only suitable for relatively slow variations. In fact, Algorithm~\ref{alg:online-meta-learning} can be applied also in setups where only some initial pilots are transmitted, followed by a long pilot-free horizon. 
Furthermore, while \cite{park2020learning,cohen2021learning} considered black-box architectures, we also show how our training algorithm can benefit from utilizing interpretable model-based architectures in the following section. % Section~\ref{sec:modular-training}.%\NirCmt{I am not sure that this description properly captures the distinction from \cite{park2020learning}. You should clarify that while the usage of meta-learning for enabling fast adaptation was considered in \cite{park2020learning}, our proposed adaptation differs from that in \cite{park2020learning} is several core aspects: First, \cite{park2020learning} focused on communication where on each coherence duration, i.e., on each channel realization, a relatively large number of pilots is transmitted followed by data symbols. Hence, \cite{park2020learning} did not consider any form of self-supervision, as training was carried out based on pilots, and both pilots and data have undergone the same channel. This implies that the approach in \cite{park2020learning} is suitable for relatively slow variations, where devoting a sufficient portion of each block to pilots does not substantially limit the spectral efficiency. Our proposed approach does not share this limitation due to its incorporation of self-supervised training and predictive meta-learning. In fact, Algorithm~\ref{alg:online-meta-learning} can be applied in a setup where only some initial pilots are transmitted, followed by a long pilot-free horizon, thus communicating in a highly spectrally efficient manner. Finally, while \cite{park2020learning} considered black-box architectures, we also show how our training algorithm can benefit from utilizing interpretable model-based architectures, as we discuss in Section~\ref{sec:modular-training}.}  . 


% \textcolor{red}{Important items to discuss:\\
% 1. Capitalize on the difference from joint learning  -- they use many past channel realizations (and typically simulated channels) to train the parameters of the deep model, we use them to adapt the {\em hyperparamters}, i.e., the optimizer, based on actual realization observed after deployment. The model itself is still adapted to the current instantaneous channel, while past data is used to optimize the optimizers. \\
% 2. We have to discuss complexity. This will inevidably arise from the reviewers and is indeed a challenge associated with our proposed design. We need to clarify that the method we propose allows DNN-aided receivers to track rapidly time-varying channels, and that these additional training rounds may be computationally complex to carry out in some applications. However, we can emphasize that the rapid growth and expected proliferation of dedicated hardware accelerators for deep learning applications, combined with the fact that training procedures are naturally prone to parallelization, indicates that more and more future digital communication devices are expected to be equipped with hardware capabilities allowing to carry out such computations in run-time.   }

==> sections_v1/model_based_detectors.tex <==
\section{Modular Training}
\label{sec:modular-training}


The training algorithm detailed in Section~\ref{sec:Hybrid Meta-Learning for Data-Driven Receivers} is applicable to any deep learning-based receiver. In this section, we \SangwooCmt{focus on deep} receivers that utilize hybrid model-based/data-driven architectures and by integrating domain knowledge in a principled manner \cite{farsad2021data, balatsoukas2019deep, shlezinger2020model}. \SangwooCmt{We adopt a modular receiver architecture to facilitate adaption to varying channels by reducing the number of parameters that require training \cite{simeone2018brief}, as compared to the end-to-end training studied in the previous section. We formulate this approach mathematically in 
Subsection~\ref{subsec:modular_training_formulation}, with Subsection~\ref{subsec:modular_training_example} providing a specific instantiation of the proposed methodology based of the DeepSIC architecture \cite{shlezinger2019deepSIC}. We end this section with a broad discussion in Subsection~\ref{subsec:modular_training_discussion}.}

% \vspace{-0.2cm}
% \subsection{Motivation}
% \label{subsec:modular_training_motivation}
% \vspace{-0.1cm}
% \SangwooCmt{To motivate modular training, we note two of the main characteristics of hybrid model-based deep symbol detectors operating in time varying channels:}
% \begin{enumerate}
%     \item Hybrid receivers often employ \textit{interpretable architectures} which carry out a principled algorithm in a learned fashion. Their interpretability means that one can typically relate their internal features with an operational quantity: Each sub-block is responsible for a concrete \SangwooCmt{role} that arises from the operation of the model-based algorithm. 
%     \item Often in communications scenarios, one can relate the channel variations to specific component in the setup. For  instance,  in  multi-user  communications  involving both  static  and  mobile  users,  channel  variations  are  often  due  to  the  movement  of  the  mobile users. Alternatively, channel variations can also be due to users joining or leaving the network. These variations, being invariant to how the receiver operates, have a great impact on the system and should be taken into consideration.
% \end{enumerate}
% \SangwooCmt{Based on these characteristics, we tailor the predictive meta-learning scheme detailed in Section~\ref{sec:Hybrid Meta-Learning for Data-Driven Receivers} for these receiver architectures, taking the above points into accounts.}

\vspace{-0.2cm}
\subsection{Modular Training}
\label{subsec:modular_training_formulation}
\vspace{-0.1cm}
A modular model-based deep receiver is partitioned into separate modules, with each module $m=1,\ldots,M$ being specified by a parameter vector $\Weights^m$. Each module generally carries out a specific functionality within the communication receiver. We note that some of these functionalities require rapid adaptation, while other can be kept unchanged over a longer time scale. Our goal is to leverage this modular structure by means of meta-learning. We refer to the set of dynamic modules requiring adaptation as $\mathcal{M}_D$ and the set of stationary modules is denoted as $\mathcal{M}_S$. To this end, we modify problem \eqref{eq:meta_2} as:

% and hyperparameter vector $\HyperParams$ can be divided into meaningful modules with parameter vectors $\Weights^m$ and hyperparameter vectors $\HyperParams^m$ for each module $m=1,\ldots,M$ (e.g., $\Weights = [\Weights^1, \ldots, \Weights^M]^\top$ and $\HyperParams = [\HyperParams^1, \ldots,\HyperParams^M]^\top$). Every module captures a specific aspect of the communication scenario. We group the modules that encounter rapid channel variations and collect the corresponding indices to form a set $\pi$; while indices of modules that exhibit static channels are denoted by the set $\pi^c$. Our goal is to employ this \emph{a priori} known information $\pi$ to find parameters and hyperparameters that enable rapid adaptation for time-varying channels; while parameters for $\pi^c$ modules remain unchanged. This can be formulated via (cf. \eqref{eq:meta_2})

\begin{multline}
    \label{eq:meta2_modular_general}
      \HyperParams_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}([\Weights^1 =  \HyperParams^1 -  \kappa^1 \nabla_{(\HyperParams^1) }\mySet{L}_{j'}(\HyperParams), \ldots,\\,\ldots, \Weights^M =  \HyperParams^M -  \kappa^M \nabla_{(\HyperParams^M) }\mySet{L}_{j'}(\HyperParams)]^\top), 
\end{multline}
where we set a learning rate $\kappa^m > 0$ for $m \in \mathcal{M}_D$ and $\kappa^m = 0$ for $m \in \mathcal{M}_S$. This approach is suitable to \cite{raghu2019rapid}, which considers a non-zero learning rate only for the last layer of a neural network, while positing that earlier layers do not need task-specific adaptations.

\SangwooCmt{Since problem \eqref{eq:meta2_modular_general} has a high computational complexity when the number of modules is large, we propose to optimize each module separately by defining proper \emph{module-wise proximal loss} $\hat{\mySet{L}}$. This loss function is often available in hybrid model-based/data-driven approaches since generally, the distinct functional role of the modules is known in advance.} 

% {Precisely, we modify \eqref{eq:meta2_modular_general} by
%and propose to meta-learn only those parameters $\Weights^m$ and hyperparameters vectors $\HyperParams^m$  whose indice is in $\pi$. For model-based architectures, we suggest to replace \eqref{eq:local_update} by
% \begin{align}
    % \label{eq:meta2_modular_general_static}
    %   \Weights_{j +1}^m  =  \mathop{\arg \min}\limits_{\Weights^m}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'})\} \in \mathcal{D}_j}     \hat{\mySet{L}}^m_{j' +1}(\Weights^m),
% \end{align}
% for modules under static channels $m \in \pi^c$;

\SangwooCmt{Specifically, in training phase, we initialize the overall parameter vector $\Weights = [\Weights^1, \ldots, \Weights^M]^\top$ for all $M$ modules by training over the obtained $T_p$ pilot blocks via \eqref{eq:meta_1} and \eqref{eq:local_update}. Then, during the evaluation phase, we adopt the dynamic modules in set $\mathcal{M}_D$ by adressing the following
\begin{align}
    \label{eq:meta2_modular_general_varying}
      \HyperParams_{j +1}^m  =  \mathop{\arg \min}\limits_{\HyperParams^m}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}    \hat{\mySet{L}}_{j' +1}(\Weights_{j'+1}^m = \HyperParams^m - \kappa^m \nabla_{\HyperParams^m}  \hat{\mySet{L}}_{j'}(\HyperParams^m)),
\end{align}
while for the static modules in $\mathcal{M}_S$, we set
% \begin{align}
% \label{eq:meta2_modular_general_static}
     $ \HyperParams_{j +1}^m  =  \Weights_j^m$.
%\end{align}
Thus, we only adapt the dynamic modules while the static module are obtained  from the training phase i.e., $\Weights_j^m = \Weights_{T_p}^m$ for $m \in \mathcal{M}_S$. The overall scheme is summarized in Algorithm~\ref{alg:modular-training}.}  

% Note that once \eqref{eq:meta2_modular_general_static} and \eqref{eq:meta2_modular_general_varying} are sufficiently learned, we can fix $\Weights^m$ for $m \in \pi^c$ and $\HyperParams^m$ for $m \in \pi$ \SangwooQuery{[is it true that online Meta-DeepSIC do not retrain $\Weights$ for static modules?]} while $\Weights^m$ for $m \in \pi$ should be adapted periodically to account for rapidly varying channels.
\SangwooCmt{In the following, we exemplify the architecture described in this section for the of \ac{mimo} detection in uplink multi-user systems via successive iteration cancellation (\ac{sic}).
}
\iffalse
\SangwooCmt{
\begin{align}
\label{eq:local_update_modular}
(\Weights^m)_{j+1}^{(t+1)} = (\Weights^m)_{j+1}^{(t)} - \eta \nabla_{\Weights^m}\mySet{L}_{j}((\Weights^m)_{j+1}^{(t)}), \: m \in \pi
 \end{align}
 \eqref{eq:meta2_modular_general} as
\begin{align}
    \label{eq:meta2_modular}
      \HyperParams^m_{j +1}  =  \mathop{\arg \min}\limits_{\HyperParams^m}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}     \mySet{L}_{j' +1}(\Weights^m =  \HyperParams^m  -  \kappa \nabla_{(\Weights^m) }\mySet{L}_{j'}(\HyperParams^m)),  \: m \in \pi.
\end{align}
}
\fi


\begin{algorithm} %!
\DontPrintSemicolon
\caption{Modular Adaptation on Incoming Block $j$ (Steps \ref{stp:onlineStart}-\ref{stp:onlineEnd} of Algorithm~\ref{alg:online-meta-learning})}
\label{alg:modular-training}
\KwIn{Step sizes $\eta, \kappa$; number of iterations $I$; threshold $\epsilon$; buffer $\mathcal{D}_{j}$; hyperparameter $\HyperParams_{j}$; rapidly-changing indices $\pi$; static modules indices $\pi^c$}
\KwOut{Hyperparameter $\HyperParams_{j+1}$; weights $\Weights_{j+1}$; buffer $\mathcal{D}_{j+1}$}
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
%{\bf Initialization} inductive bias $\HyperParams_1$ and ViterbiNet $\Weights_1$ \\
%{\bf Initialization} buffer $\mathcal{D}_1$ as empty, i.e., $\mathcal{D}_1 \leftarrow [ \hspace{0.2cm} ]$ \\
%\For{$j = 1,2,\ldots$}{
\nonl\texttt{Online predictive meta-learning (every $F$ blocks)}\;
\SangwooCmt{
\For{$m = 1,\ldots,M$}{
\uIf{$m \in \pi$ }{ 
Set $\HyperParams_{j+1}^{(0)} = \HyperParams^m_j$\;
\For{$i=0,1,\ldots$}{
\label{stp:Random2} Randomly select block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})\in \mathcal{D}_{j}$\; % except for the last block in the buffer $\mathcal{D}_j$\\  
      {\uIf{$(\myVec{s}_{j'}, {\myVec{y}}_{j'})\notin \mathcal{D}_{j}$}{
  go back to line \ref{stp:Random2} \tcp*{invalid data for meta-learning}
  }
  }
  Set $\hat{\HyperParams}^{(0)} = \HyperParams_{j+1}^{(i)}$\;
    \For{$t=0,1,\ldots,I-1$}{
   Use block $(\myVec{s}_{j'}, {\myVec{y}}_{j'})$ to compute \tcp*{support task}
      \begin{equation*}
\hat{\Weights} = \hat{\HyperParams}^{(t)} -\eta\nabla_{\hat{\HyperParams}^{(t)}} \hat{\mySet{L}}_{j'}(\Weights^m=\hat{\HyperParams}^{(t)}). \end{equation*} \;
    Use subsequent block $(\myVec{s}_{j'+1}, {\myVec{y}}_{j'+1})$ to update \tcp*{query task}
  \begin{equation*}
\hat{\HyperParams}^{(t+1)} = \hat{\HyperParams}^{(t)} - \kappa^m \nabla_{\hat{\HyperParams}^{(t)} }\hat{\mySet{L}}_{j'+1}(\Weights^m =\hat{\Weights}). 
\end{equation*}
    }
    Update hyperparameter as $\HyperParams_{j+1}^{(i+1)} =\hat{\HyperParams}^{(I)}$ \tcp*{meta-update}
}
Set hyperparameter $\HyperParams^m_{j+1} =\HyperParams_{j+1}^{(i+1)}$ \tcp*{update the hyperparameter}
}
\uElse{ 
      Set hyperparameter $\HyperParams^m_{j+1} =\Weights^m_{j}$ \tcp*{copy the $m$th hyperparameter}
  }
}}

\nonl\texttt{Online learning (on each block)} \;
{\uIf{(Pilot) or (Decoding is correct)}{
 \For{$m \in \pi$}{Train $\Weights^m_{j+1}$ with $({\myVec{s}}_j, {\myVec{y}}_j)$ and initialization $\HyperParams^m_{j+1}$  via \eqref{eq:meta_1} \tcp*{update} }
 \For{$m \in \pi^c$}{
 $\Weights^m_{j+1} \leftarrow \Weights^m_j$ \tcp*{no update for static} }
  }
  \uElse{ 
      $\Weights_{j+1} \leftarrow \Weights_j$ \tcp*{no update}
  }
  $\mathcal{D}_{j+1}\leftarrow \mathcal{D}_{j}$ \tcp*{keep buffer}
  }
 %}
\end{algorithm}


% \begin{align}
%       \HyperParams^*  =  \mathop{\arg \min}\limits_{\HyperParams = [\HyperParams^1, \ldots, \HyperParams^M]^\top}     \mathbb{E}_{P_\tau} \left[ \mySet{L}_{\tau}(\Weights =  [\HyperParams^1  -  \kappa^1 \nabla_{\HyperParams^1 }\mySet{L}_{\tau}(\HyperParams),\ldots, \HyperParams^M  -  \kappa^M \nabla_{\HyperParams^M }\mySet{L}_{\tau}(\HyperParams)]^\top)\right],
%       \label{eq:general_anil}
% \end{align}
% Our approach, coined modular training, seeks to jointly exploit these properties for  setups  where  the  interpretable  nature  of  the  deep  receiver  sub-blocks  can  be  related  with the  components  of  the  channel  where  variations  originate. Specifically, as hybrid model-based/data-driven receivers can often divided into meaningful sub-blocks, we wish to train only those that relate to a specific time-varying component of the underlying channel. 
% We next show how to apply modular training in uplink \ac{mimo} systems, employing the DeepSIC receiver \cite{shlezinger2019deepSIC}.

\vspace{-0.2cm}
\subsection{Modular DeepSIC Receiver}
\label{subsec:modular_training_example}
\vspace{-0.1cm}
We focus on a special case of the generic  model detailed in Subsection~\ref{subsec:Channel}, in which the channel is memoryless ($L=1$), while the receiver has $N>1$ antennas and it communicates with $K>1$ users. A single user with index $k'\in \{1,\ldots,K\}$ is mobile, while the remaining are static. We assume that the receiver knows which of the users is mobile and which is static, i.e., it has prior knowledge of $k'$. Such scenario arise, for instance, in a traffic monitoring infrastructure, where a multi-antenna \acl{bs} communicates with both static road-side units and mobile vehicles. Communication can be directly obtained  from the method described here.

We adopt the DeepSIC receiver proposed in \cite{shlezinger2019deepSIC} as a modular receiver architecture. DeepSIC is derived from iterative \ac{sic} \cite{choi2000iterative}, which is a \ac{mimo}  detection method combining multi-stage interference cancellation with soft decisions. For brevity, we omit here the subscripts representing the time instance and the block index, using $\myVec{Y}$ to denote the random channel output and $\myVec{S}=[\myVec{S}_1,\ldots,\myVec{S}_K]^T$ the transmitted symbols. 
DeepSIC operates in $Q$ iterations, refining an estimate of the conditional \acl{pmf} of $\myVec{S}_k$, denoted by $\hat{\myVec{p}}_{k}^{(q)}$ where $q$ is the iteration number. This estimate   is generated for every symbol $k \in \{1,2,\ldots, K\}$ by using the corresponding estimates of the interfering symbols $\{S_l\}_{l \neq k}$ obtained in the previous iteration $\{\hat{\myVec{p}}_{\tilde{k}}^{(q-1)}\}_{\tilde{k}\neq k}$. Iteratively repeating this procedure refines the conditional distribution estimates, allowing the detector to accurately recover each symbol from the output of the last iteration.  This iterative procedure is illustrated in Fig.~\ref{fig:SoftIC}(a). 

\SangwooCmt{In DeepSIC, the interference cancellation and soft decoding steps are implemented with \acp{dnn}. The soft estimate of the symbol transmitted by $k$th user in the $q$th iteration is done by a \ac{dnn} based classifying module with parameters $\Weights^{k,q}$. The output of the \ac{dnn} module with parameters $\Weights^{k,q}$ is a soft estimate of the symbol of the $k$th user. The set $\Weights = \{\Weights^{k,q}\}$ describes the model parameters. The resulting \ac{dnn}-aided receiver, illustrated in Fig.~\ref{fig:SoftIC}(b), was shown in \cite{shlezinger2019deepSIC}  to accurately carry out \ac{sic}-based \ac{mimo} detection in complex channel models.} 

\begin{figure}
	\centering
	\includegraphics[width = 0.9\columnwidth]{fig/DeepSIC1.png}
	\vspace{-0.4cm}
	\caption{(a) Iterative soft interference cancellation, and (b) the \ac{dnn}-aided DeepSIC.}
	%	\vspace{-0.4cm}
	\label{fig:SoftIC}
\end{figure}

\SangwooCmt{We employ modular training as described in Algorithm~\ref{alg:modular-training}. DeepSIC uses $M=K \cdot Q$ modules, with the $(k,q)$-th module detecting the symbol of user $k$ at iteration $q$. Since only user $k'$ is moving, we define the set of dynamic modules as $\mathcal{M}_D = \{(k',q)\:|\:q\in\{1,\ldots,Q\}\}$, with all other modules being static. We define the module-wise proximal loss \eqref{eq:meta2_modular_general_varying} for module $k$ at iteration $q$ as the cross entropy
\begin{align}
   \hat{\mySet{L}}_{j}(\Weights^{k,q}) = -\sum_{i=1}^{\Blklen}\log \hat{P}_{\Weights^{k,q}}(\myVec{y}_{i,j}, \{ \hat{\myVec{p}}_{i,j}^{\tilde{k},q-1} \}_{\tilde{k}\neq k} | \myStateR_{i,j}),
\end{align}
where $\hat{\myVec{p}}^{\tilde{k},q-1}$ is the estimated symbol probability for the $\tilde{k}$th user at iteration $q-1$. The module-wise parameter vector $\Weights_{j+1}^{k,q}$ for each $(k,q)\in \mathcal{M}_D$ is obtained from $I$ gradient descent iterations
\begin{align}
    \Weights_{j+1}^{k,q} = \HyperParams^{k,q}_{j+1} - \kappa^{k,q} \nabla_{ \HyperParams^{k,q}}\hat{\mySet{L}}_{j}(\Weights^{k,q}_{j+1})
    \label{eq:meta3_modular_general_varying_deepsic}
\end{align}
with $\HyperParams^{k,q}_{j+1}$ being optimized via \eqref{eq:meta2_modular_general_varying}, namely,
\begin{align}
    \label{eq:meta2_modular_general_varying_deepsic}
      \HyperParams_{j +1}^{k,q}  =  \mathop{\arg \min}\limits_{\HyperParams^{k,q}}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}    \hat{\mySet{L}}_{j' +1}(\Weights^{k,q} = \HyperParams^{k,q} - \kappa^{k,q} \nabla_{ \HyperParams^{k,q}} \hat{\mySet{L}}_{j'}(\HyperParams^{k,q})).
\end{align}
We note that problem \eqref{eq:meta2_modular_general_varying_deepsic} uses all previous data up to time $j+1$; while \eqref{eq:meta3_modular_general_varying_deepsic} only uses only data from block $j$ for the local update.}

% \SangwooQuery{Precisely, we take module-wise proximal loss for the module $k$ at iteration $q$ as
% \begin{align}
%   \hat{\mySet{L}}_{j+1}^{k,q}(\Weights) = -\log \hat{P}_{\Weights}^{k,q}({y}_{j+1}, \{ \hat{p}^{\tilde{k},q-1} \}_{\tilde{k}\neq k} | s_{j+1}),
% \end{align}
% where $\hat{p}^{\tilde{k},q-1}$ is the output (estimated symbol probability for the user $\tilde{k}$) of the module $\tilde{k}$ at iteration $q-1$ which is evaluated via $\Weights_{j+1}^{\tilde{k},q-1}$ obtained from previous iteration as (cf. \eqref{eq:meta2_modular_general_static})
% \begin{align}
%     \label{eq:meta2_modular_general_static_deepsic}
%       \Weights_{j +1}^{\tilde{k},q-1}  =  \mathop{\arg \min}\limits_{\Weights^m}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'})\} \in \mathcal{D}_j}     \hat{\mySet{L}}^{\tilde{k},q-1}_{j' +1}(\Weights^m),
% \end{align}
% for $\tilde{k} \neq k'$ while for $\tilde{k}=k'$, $\Weights_{j+1}^{k',q-1}$ is optimized through 
% \begin{align}
%     \Weights_{j+1}^{k',q-1} = \HyperParams^{k'}_{j+1} - \kappa^{k'} \hat{\mySet{L}}_{j}^{k',q-1}(\HyperParams^{k'}_{j+1})
%     \label{eq:meta3_modular_general_varying_deepsic}
% \end{align}
% with $\HyperParams^{k'}_{j+1}$ being optimized from
% (cf. \eqref{eq:meta2_modular_general_varying})
% \begin{align}
%     \label{eq:meta2_modular_general_varying_deepsic}
%       \HyperParams_{j +1}^{k'}  =  \mathop{\arg \min}\limits_{\HyperParams^{k'}}     \sum\limits_{\{(\myVec{s}_{j'}, {\myVec{y}}_{j'}), (\myVec{s}_{j'+1}, {\myVec{y}}_{j' +1})\} \in \mathcal{D}_j}    \hat{\mySet{L}}^{k',q-1}_{j' +1}(\Weights_{j'+1}^{k'} = \HyperParams^{k'} - \kappa^{k'} \hat{\mySet{L}}_{j'}(\HyperParams^{k'})).
% \end{align}
% It is worth noting that \eqref{eq:meta2_modular_general_static_deepsic} uses all the previous data set up to current time $j+1$; while \eqref{eq:meta3_modular_general_varying_deepsic} only use previous data set at time $j$ since the hyperparameter for $k'$ is designed to be adapted for the next time $j+1$.} \SangwooCmt{The overall meta-learning for DeepSIC is detailed in Algorithm~\ref{alg:modular-training}.\SangwooQuery{Similar to algorithm 3 in Nir's original DeepSIC paper, I guess? }}

\vspace{-0.2cm}
\subsection{Discussion}
\label{subsec:modular_training_discussion}
\vspace{-0.1cm}
Modular training via Algorithm~\ref{alg:modular-training} exploits the model-based structure of hybrid \ac{dnn} receivers to further accelerate the training on short blocks and improve adaptation. This follows from the fact that Algorithm~\ref{alg:modular-training} only trains a  portion  of  the  overall  network, i.e., it uses the same data as in Algorithm~\ref{alg:online-meta-learning} while adapting less parameters, thus gaining in convergence speed and accuracy of the trained model. The exact portion of the overall parameters is  dictated  by  the  ratio  of  the mobile users to the overall users in the network. The smaller the ratio is, the more one can benefit from modular training. We validate the benefits of modular training in Subsection~\ref{subsec:modular-training} and show that this approach can decrease the average \ac{ber} significantly. Indeed, our experimental results demonstrate that the proposed approach successfully translates the prior knowledge on the nature of  the  variations  into  improved  performance,  particularly  when  dealing  with  short  blocks,  i.e. short coherence duration of rapidly varying channels. 

This modular training approach can be viewed as a form of transfer learning, as it trains online only parts of the parameters. Yet, it is specifically tailored towards interpretable architectures, adapting internal sub-modules of the overall network, as opposed to the common transfer learning approach of retraining the output layers. For instance, the suggested method trains the sub-modules associated with all mobile users separately in an iterative fashion, building upon the fact that each module $\Weights^{k,q}$ should produce a soft estimate of $\myVec{S}_k$.  Modular training can also be enhanced to carry out some final tuning of the overall network since, e.g., the channels of the mobile users is expected to also affect how their interference is canceled when recovering the remaining users via the sub-modules which are not adapted online.  
Finally, it is noted that this approach relies on knowledge of the mobile user, and thus incorrect knowledge of $k'$ is expected to affect the accuracy of the trained receiver.  We  leave  the  study  of  the resilience of modular training and the aforementioned extensions for future work.

==> sections_v1/results.tex <==
\section{Numerical Evaluations}
\label{sec:Simulation}
\vspace{-0.1cm} 
In this section we numerically evaluate the proposed online adaptation scheme in finite-memory \ac{siso} chanels and in memorylesss multi-user \ac{mimo} setups\footnote{The source code used in our experiments is available at \href{https://github.com/tomerraviv95/MetaDeepSIC}{https://github.com/tomerraviv95/MetaDeepSIC}}. 
We first describe the receivers compared in our experimental study, detailing the architectures in Subsection~\ref{subsec:simEqualizers} and the training methods in Subsection~\ref{subbsec:Training Methods}. Then, we present the main simulation results for evaluating online meta-learning on linear synthetic channels, non-linear synthetic channels, and channels obeying the COST 2100 model in Subsections~\ref{subsec:synth_simulation_results} to \ref{subsec:cost_simulation_results}. Finally, we numerically evaluate Algorithm~\ref{alg:modular-training} which combines online meta-learning with the modular training in Subsection~\ref{subsec:modular-training}.
%, as well as the effect of our learning schemes on pilot efficiency, in Subsections~\ref{subsec:modular-training} and \ref{subsec:pilot-training}, respectively.


%-----------------------------------
%	ViterbiNet
%-----------------------------------
% \subsection{ViterbiNet}
% \label{subsec:ViterbiNet}


% Following the channel definition of Subsection~\ref{subsec:SISOChannel}, the Viterbi equalizer solves the maximum likelihood sequence detection problem
% \begin{align}
% \hat{\myVec{s}}_j   
% &= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i,j}\right)\right\}.
% \label{eqn:ML3} 
% \end{align}	
% In particular,  \eqref{eqn:ML3} is solved recursively via dynamic programming, by  iteratively updating a {\em path cost} $c_i(\myStateR)$ for each state $\myStateR\in \bar{\mySet{S}}$ for $i=1,2,\ldots,B$. ViterbiNet implements Viterbi detection in a data-driven fashion by training a \ac{dnn} to provide a parametric estimate of the likelihood function $\hat{P}_{\Weights}\left( \myVec{y}  |  \myStateR\right)$. Meta-ViterbiNet \cite{raviv2021meta} applies Algorithm~\ref{alg:online-meta-learning} to ViterbiNet, leading to higher adaptivity over fast channel variations.

%-----------------------------------
%	Evaluated Equalizers
%-----------------------------------
\vspace{-0.4cm}
\subsection{Evaluated Receivers}
\label{subsec:simEqualizers}
The receiver algorithms used in our experimental study vary based on the considered settings:
%\vspace{-0.1cm}
\subsubsection{Finite-Memory \ac{siso} Channels}
We compare two  \ac{dnn}-aided receivers for \ac{siso} settings:
\begin{itemize}
    \item The ViterbiNet equalizer, proposed in \cite{shlezinger2019viterbinet}, which is a \ac{dnn}-aided Viterbi detector for finite-memory channels of the form \eqref{eqn:ChModel1} \cite{viterbi1967error}. The Viterbi equalizer (from which ViterbiNet originates) solves the maximum likelihood sequence detection problem
\begin{align}
\hat{\myVec{s}}_j   
&= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i-\Mem+1,j},\ldots, \myStateR_{i,j}\right)\right\}.
\label{eqn:ML3} 
\end{align}	
    ViterbiNet computes each log likelihood using a  \ac{dnn} that requires no  knowledge of the channel  distributions $ \Pdf{\myVec{Y}_j |  \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}$. This internal \ac{dnn} is implemented using three fully-connected layers of sizes $1\times 100$, $100\times 50$, and $50 \times |\mySet{S}|^\Mem$, with activation functions set to sigmoid (after first layer), ReLU (after second layer), and softmax output layer.
    %sigmoid and ReLU activations, respectively, and a softmax output layer. 
    \item A recurrent neural network  symbol detector, comprised of a sliding-window \ac{lstm} classifier with two hidden layers of 256 cells and window size $\Mem$, representing a black-box \ac{dnn} benchmark \cite{tandler2019recurrent}.
\end{itemize}
%
The Viterbi equalizer  with complete knowledge of the channel is used as a baseline method.

\subsubsection{Memoryless \ac{mimo} Channels}
We evaluate two  \ac{dnn}-aided \ac{mimo}  receivers:
\begin{itemize}
    \item The DeepSIC receiver detailed in Subsection~\ref{subsec:modular_training_example}. The building blocks of DeepSIC are implemented using three fully-connected layers:  An $(N + K - 1) \times 100$ first layer, a $100 \times 50$ second layer, and a $50 \times |\mySet{S}|$ third layer, with a sigmoid and a ReLU intermediate activation functions, respectively. The number of iterations is set to $Q=5$.  
    %sigmoid and ReLU activations, respectively, and a softmax output layer. 
    \item A ResNet10 black-box neural network, which is based on the  DeepRX architecture proposed in \cite{honkala2021deeprx}. The architecture is comprised of 10 residual blocks \cite{he2016deep}, each block has two convolutional layers with 3x3 kernel, one pixel padding on both sides, and no bias terms, with a ReLU  in-between. 
    A 2D batch normalization follows each convolutional layer.
\end{itemize}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_train_channel.png}
    \caption{Synthetic training channel.}
    \label{fig:synthetic_train_channel}
    \end{subfigure} 
    %
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_test_channel.png}
    \caption{Synthetic test channel.}
    \label{fig:synthetic_test_channel}
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/cost_channel.png}
    \caption{COST 2100 channel.}
    \label{fig:COSTChannel} 
    \end{subfigure}
    \caption{Examples of time-varying channels: channel coefficients versus block index.}
    \figSpace
    \label{fig:channels} 
 %   \vspace{-0.1cm}
\end{figure*}


\subsection{Training Methods}
\label{subbsec:Training Methods}
Before the test phase begins, we generate a set $\mathcal{D}_0$ of $T_p$ pilot blocks. We then use the following methods for adapting the deep receivers:
\begin{itemize}
    \item {\em Joint training}: The \ac{dnn} is  trained on $\mathcal{D}_0$ only by minimizing the empirical cross-entropy loss, and no additional training is performed in the test phase.
    \item {\em Online training} \cite{shlezinger2019viterbinet}: The \ac{dnn} is initially trained  on $\mathcal{D}_0$ by minimizing the empirical cross-entropy loss. Then, during test, the \ac{dnn} parameter vector $\Weights_j$ is re-trained on each successfully decoded data block and on each incoming pilot block as specified in \eqref{eq:local_update}, using $\Weights_{j}$ in lieu of $\HyperParams_{j+1}$. %, using a fixed non-optimized inductive bias $\HyperParams$.
    \item {\em Online meta-learning}: 
    Here, we first meta-train $\HyperParams_0$ with $\mathcal{D}_0$ similar to \eqref{eq:meta_2} as
    \begin{align*}
    %\label{eq:offline_meta}
     \HyperParams_{0} = \mathop{\arg \min}_{\HyperParams} \sum_{\{(\myVec{s}_{ j'}, {\myVec{y}}_{ j'}), (\myVec{s}_{ j'+1}, {\myVec{y}}_{ j'+1})\} \in \mathcal{D}_0}    \mySet{L}_{ j'+1}(\Weights = \HyperParams  -  \kappa \nabla_{ \HyperParams }\mySet{L}_{ j'}(\Weights =\HyperParams)).
\end{align*}
    
    %To this end, meta-training splits the buffer $\mathcal{D}_0$ into following-words pairs as $(\boldsymbol{y}^B_0,\boldsymbol{y}^B_1),\ldots,(\boldsymbol{y}^B_{T_t-2},\boldsymbol{y}^B_{T_t-1})$. The first word of each pair $\boldsymbol{y}^B_{2n}$ is used for the local update (\ref{eq:local_update}), while the second word $\boldsymbol{y}^B_{2n+1}$ is used for the global update calculation as in
	%\begin{align}
	%\label{eq:meta_2_pred_offline}
	 % \mathop{\arg \min}_{\HyperParams_0} \sum_{\text{odd }j} \mySet{L}_j(\Weights= \HyperParams_0 - \eta \nabla_{ \HyperParams_0}\mySet{L}_{j-1}( \HyperParams_0)).
	%\end{align}
	This  process yields the initial hyperparameters $\HyperParams_0$. 
	Then, during test,   Algorithm~\ref{alg:online-meta-learning} is used with online learning every block and online meta-learning every $F=5$ blocks. The number of online meta-learning updates   equals that of online training, thus inducing a relative small overhead due to its additional computations. The combination of online meta-learning with ViterbiNet is henceforth referred to as {\em Meta-ViterbiNet}, while the DeepSIC receiver trained with this approach is coined {\em Meta-DeepSIC}.
\end{itemize}


%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{Linear Synthetic Channel Results}
\label{subsec:synth_simulation_results}
\vspace{-0.1cm}
We begin by evaluating Algorithm~\ref{alg:online-meta-learning} on synthetic time-varying linear channels with additive Gaussian noise, considering  a finite-memory \ac{siso} setting and a memoryless \ac{mimo} setup.
%
\subsubsection{\ac{siso} Finite-Memory Channels} 
%We refer to the combination of the ViterbiNet equalizer and online meta-training as Meta-ViterbiNet. 
Recalling Fig.~\ref{fig:transmission}, we transmit $T_p=T_d=300$ blocks comprised of $\Blklen = 136$ symbols, i.e., a relatively short coherence duration for the time-varying channel. Each block includes $120$ information bits, encoded using a \acl{rs} [17,15] code with two parity symbols with \ac{bpsk} modulation, i.e., $\mySet{S} = \{\pm 1\}$.  %The online meta-learning in Algorithm \ref{alg:online-meta-learning} is executed every $K=5$ blocks. 

We consider a linear Gaussian channel, whose input-output relationship is given by
\begin{equation}
\label{eqn:Gaussian}
\myY_{i,j} = \sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j},
\end{equation}
where $\myVec{h}_j = [h_{0,j},\ldots,h_{\Mem-1,j}]^T$ are the real channel taps, and $w_{i,j}$ is \acl{awgn} with variance $\sigma^2$. The channel memory is $\Mem = 4$ with the taps $\{h_{l,j}\}$  generated using a synthetic model representing oscillations of varying frequencies. 
%
Here,  the signals received during the pilots used for initial training $(\mathcal{D}_0)$ are subject to the time-varying channel whose taps are illustrated in Fig.~\ref{fig:synthetic_train_channel}; while we use the taps  in Fig.~\ref{fig:synthetic_test_channel} for testing. This channel represents oscillations of varying frequencies. %, where  the periods of the taps become aligned as the noise subsides. 


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_block.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:SyntheticBERvsBlock}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_ber_versus_snr.png}
    \caption{Coded \ac{ber} after 300 blocks vs. SNR.}
    \label{fig:SyntheticBERvsSNR}
    \end{subfigure}
    %
    \caption{\ac{siso} synthetic linear Gaussian channel, $\Blklen = 136$.}
    \label{fig:SyntheticBER} 
    \figSpace
\end{figure*}

In Fig.~\ref{fig:SyntheticBERvsBlock} we plot the evolution of the average coded \ac{ber} of the considered receivers when the \ac{snr}, defined as $1/\sigma^2$, is set to $12$ dB. Fig.~\ref{fig:SyntheticBERvsBlock} shows that Meta-ViterbiNet significantly outperforms its benchmarks, demonstrating the gains of the proposed online meta-learning training and its suitability when combined with receiver architectures utilizing relatively compact \acp{dnn}. In particular, it is demonstrated that each of the ingredients combined in Meta-VitebiNet, i.e., its model-based architecture, the usage of self-supervision, and the incorporation of online meta-learning, facilitates operation in time-varying conditions: The ViterbiNet architecture consistently outperforms the black-box \ac{lstm} classifier; Online training yields reduced \ac{ber} as compared to joint learning; and its combination with meta-learning via Algorithm~\ref{alg:online-meta-learning} yields the lowest \ac{ber} values.  
%
To further validate that these gains also hold for different \acp{snr}, we show in Fig.~\ref{fig:SyntheticBERvsSNR} the average coded \ac{ber} of the evaluated receivers after 300 blocks, averaged over 5 trials. We observe in Fig.~\ref{fig:SyntheticBERvsSNR} that for \ac{snr} values larger than $8$ dB, Meta-ViterbiNet consistently achieves the lowest  \ac{ber} values among all considered data-driven receivers, with gains of up to 0.5dB over the online training counterpart.





\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_1.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:SyntheticBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_2.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:SyntheticBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} synthetic linear Gaussian channel, $\Blklen = 152$.}
    \label{fig:SyntheticBERMIMO} 
    \figSpace
\end{figure*}

\subsubsection{Memoryless MIMO Channels} 
For the \ac{mimo} setting, use $T_p=T_d=50$ blocks. The block length is set to $\Blklen = 152$ symbols, encoding 120 information bits with \acl{rs} [19,15] code. The input-output relationship of a the memoryless Gaussian \ac{mimo} channel is given by
\begin{equation}
\label{eqn:GaussianMIMO}
\myY = \myMat{H}\myS + \myVec{W},
\end{equation}
where $\myMat{H}$ is a known deterministic $N\times K$ channel matrix, and $\myVec{W}$ consists of $N$ i.i.d Gaussian \acp{rv}.  
We set the number of users and antennas to $N=K=4$. The channel matrix $\myMat{H}$ models spatial exponential decay, and its entries are given by
$\left( \myMat{H}\right)_{n,k} = e^{-|n-k|}$, for each $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$.  The transmitted symbols are generated from a \ac{bpsk} constellation in a uniform i.i.d. manner, i.e., $\mathcal{S}=\{\pm 1\}$.

The numerical results for the memoryless Gaussian channel \eqref{eqn:GaussianMIMO} are depicted in Fig.~\ref{fig:SyntheticBERMIMO}.
Note that Fig.~\ref{fig:SyntheticBERvsBlockMIMO} shows the average coded \ac{ber} of the receivers for ${\rm SNR} = 14$ dB for a single trial, while Fig.~\ref{fig:SyntheticBERvsSNRMIMO} shows a sweep over a range of \ac{snr} values after 50 blocks, averaged over 10 trials. Similarly to Meta-ViterbiNet in the finite-memory \ac{siso} setting, Meta-DeepSIC outperforms all other training methods in medium to high SNRs. Here, the black-box architectures perform quite poorly, unable to compete with the model-based architecture of DeepSIC due to short blocklengths and the highly limited volumes of data used for training. Training DeepSIC with Algorithm~\ref{alg:online-meta-learning} outperforms the joint training approach with gains of up to 1dB, and with gains of 1.5dB over online training, which notably struggles in tracking such rapidly time-varying and challenging conditions.


\vspace{-0.4cm}
\subsection{Non-Linear Synthetic Channel Results}
\label{subsec:syntNL_simulation_results}
\vspace{-0.1cm}
Next, we evaluate the proposed online meta-learning scheme in non-linear synthetic channels, where one can greatly benefit from the model-agnostic nature of \ac{dnn}-aided receivers. 


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_block_siso.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:NonLinearSyntheticBERvsBlockSISO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/non_linear_synth_ber_versus_snr_siso.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:NonLinearSyntheticBERvsSNRSISO}
    \end{subfigure}
    %
    \caption{\ac{siso} synthetic non-linear Gaussian channel, $\Blklen = 136$.}
    \label{fig:NonLinearSyntheticBERSISO} 
    \figSpace
\end{figure*}

\subsubsection{\ac{siso} Finite-Memory Channels} To check the robustness of our method in a non-linear case, we generate a non-linear channel by applying a non-linear transformation to synthetic channel in \eqref{eqn:Gaussian}. The resulting finite-memory \ac{siso} channel is give by
\begin{equation}
\label{eqn:Gaussian1}
\myY_{i,j} =\tanh{\Big(C \cdot \Big(\sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j}\Big)\Big)}.
\end{equation}
This operation may represent, e.g., non-linearities induced by the receiver acquisition hardware. The hyperparameter $C$ stands for a power attenuation at the receiver, and chosen empirically as $C=\frac{1}{2}$. All other hyperparameters and settings are the same as those used in the previous subsection. This simulation shows a consistent gain of around $0.75$dB over the SNRs with values of $8$dB - $12$dB, as observed in Fig.~\ref{fig:NonLinearSyntheticBERSISO}.

\subsubsection{Memoryless \ac{mimo} Channels} Similarly to the \ac{siso} case, we simulate a non-linear \ac{mimo} channel from \eqref{eqn:GaussianMIMO} via
\begin{equation}
\label{eqn:Gaussian2}
\myY = \tanh{\Big(C \cdot\Big(\myMat{H}\myS + \myVec{W}\Big)\Big)}.
\end{equation}
Similarly, $C=\frac{1}{2}$ and the remaining simulation settings are chosen as in Subsection~\ref{subsec:synth_simulation_results}. The numerical results for this channel are illustrated in Fig.~\ref{fig:NonLinearSyntheticBERMIMO}, showing that the superiority of our approach is maintained in non-linear setups. The right part shows an average over 20 trials, while the left graph corresponds to an exemplary trial. In particular, we note that gains of up to 0.5dB in high SNRs are achieved compared with online training, while the gap from joint method is around 0.25dB. Here, our gain becomes apparent as the SNR increases.


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_3.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:NonLinearSyntheticBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_4.png}
    \caption{Coded \ac{ber} after 50 blocks vs. SNR.}
    \label{fig:NonLinearSyntheticBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} synthetic non-linear Gaussian channel, $\Blklen = 152$.}
    \label{fig:NonLinearSyntheticBERMIMO} 
    \figSpace
\end{figure*}

%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{COST 2100 Channel Results}
\label{subsec:cost_simulation_results}
\vspace{-0.1cm}

Next, we consider channels generated using the COST 2100 geometry-based stochastic channel model \cite{liu2012cost}. This model is widely used in indoor wireless communications.

% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/test_8x8_cost_ant1.png}
%     \caption{Antenna 1 channel.}
%     \label{fig:cost_channel_antenna1}
%     \end{subfigure}
%     %
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/test_8x8_cost_ant2.png}
%     \caption{Antenna 2 channel.}
%     \label{fig:cost_channel_antenna2}
%     \end{subfigure}
%     %
%     \caption{\ac{mimo} COST 2100 channels.}
%     \label{fig:CostBER} 
%     \figSpace
% \end{figure*}

\subsubsection{\ac{siso} Finite-Memory Channels} In particular, we generate each realization of the taps using an indoor hall $5$GHz setting with single-antenna elements. We use the same block length and number of error-correction symbols, as well as the same initial training set $\mySet{D}_0$ as in the synthetic model. This setting may represent a user moving in an indoor setup while switching between different microcells. Succeeding on this scenario requires high adaptivity since there is considerable mismatch between the train and test channels. The test is carried out using a sequence of difference realizations illustrated in Fig.~\ref{fig:COSTChannel}, whereas the initial training still follows the taps illustrated in Fig.~\ref{fig:synthetic_train_channel}. The two main figures, Fig.~\ref{fig:SISOcostBERvsBlock} and Fig.~\ref{fig:SISOcostBERvsSNR} illustrate gains of up to 0.6dB by using our scheme compared to other methods. 


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/costBERvsBlock.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 12$ dB.}
    \label{fig:SISOcostBERvsBlock}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_ber_versus_snr.png}
    \caption{Coded \ac{ber} after 300 blocks vs. SNR.}
    \label{fig:SISOcostBERvsSNR}
    \end{subfigure}
    %
    \caption{\ac{siso} COST 2100 channel, $\Blklen = 136$.}
    \label{fig:SISOCostBER} 
    \figSpace
\end{figure*}

\subsubsection{Memoryless \ac{mimo} Channels} For the current \ac{mimo} setting, we compose the test channels from only $T_p=T_d=40$ blocks and increase the number of users and antennas to $N = K = 8$. To simulate the channel matrix $\myMat{H}$, we follow the above \ac{siso} description and create $8 \times 8 = 64$ \ac{siso} COST 2100 channels; Each simulated channel corresponds to a single entry $\left( \myMat{H}\right)_{n,k}$ with $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$. Moving to results, one may observe the respective graphs Fig.~\ref{fig:costBERvsBlockMIMO} and Fig.~\ref{fig:costBERvsSNRMIMO}, which show an unusual gain of up to 2dB approximately, as the joint and online methods are unable to compete with the proposed meta approach. The results here are averaged over 20 trials.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_5.png}
    \caption{Coded \ac{ber} vs. block index, ${\rm SNR} = 14$ dB.}
    \label{fig:costBERvsBlockMIMO}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_6.png}
    \caption{Coded \ac{ber} after 40 blocks vs. SNR.}
    \label{fig:costBERvsSNRMIMO}
    \end{subfigure}
    %
    \caption{\ac{mimo} COST 2100 channel, $\Blklen = 152$.}
    \label{fig:CostBERMIMO} 
    \figSpace
\end{figure*}



\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_7.png}
    \caption{Synthetic linear channel.}
    \label{fig:synth_modular_online}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/figure_8.png}
    \caption{COST 2100 channel.}
    \label{fig:cost_modular_online}
    \end{subfigure}
    %
    \caption{Modular Training - Coded \ac{ber} vs. \ac{snr}, $\Blklen = 152$.}
    \label{fig:ModularTrainingOnline} 
    \figSpace
\end{figure*}

\subsection{Modular Training Results}
\label{subsec:modular-training}
% As discussed before, our approach is best utilized with the model-based architectures. This is due to the model-based structure of the receiver, having fewer parameters than model-free receivers. This fact permits quick adaption with small block size. To further exploit the interpretable structure of the model, we employ a new modular training scheme as explained in Section~\ref{sec:modular-training}. 
To evaluate the modular training methods proposed in Section~\ref{sec:modular-training}, we next consider a multi-user \ac{mimo} setting. Here, the temporal variations stem from the fact that only a single user is changing ($k'=2$), with the other ones being static. The receiver uses DeepSIC, and has domain knowledge regarding the identity of the dynamic user. We numerically compare the gains of exploiting this knowledge using Algorithm~\ref{alg:modular-training}, as well as the individual gains of combining modular training with predictive meta-learning compared with online adapting solely the network weights.

% We apply the modular training method: Training the neural networks of a single given user, as described in Subsection~\ref{subsec:modular_training_formulation} and Subsection~\ref{subsec:modular_training_example}.
\SangwooCmt{Fig.~\ref{fig:ModularTrainingOnline} shows the two compared methods -- online-training and (predictive) online-meta training, executed either with or without modular training (Algorithm~\ref{alg:modular-training}) for the synthetic linear channel (Fig.~\ref{fig:synth_modular_online}) and the COST 2100 channel (Fig.~\ref{fig:cost_modular_online}). We also plot the joint training method for completeness. 
Observing the plotted curves, one may observe that our modular meta-training achieves superior results compared to the other methods. As depicted in Fig.~\ref{fig:synth_modular_online}, one may gain additional 0.3dB under the meta-learning scheme by employing the modular training approach, for low and high \ac{snr} values. In medium \ac{snr}, one is expected to achieve similar results to the non-modular method. On the other hand, in Fig.~\ref{fig:cost_modular_online} one may benefit significantly by using the combined approach, due to the rapid variations of the channel. Specifically, the modular gains appear in low to medium \ac{snr}, while the gains of the meta-learning stage appear for the higher SNR values. The gain in both scenarios for the two-stage approach versus the simple online training is up to 2.5dB. These results indicate the gains of our two-stage approach, and show that Algorithm~\ref{alg:modular-training} allows to translate the interpretable modular architecture of DeepSIC into improved online adaptation in the presence of temporal variations due to a combination of mobile and static users.}

% \subsection{Pilots Efficiency} 
% \label{subsec:pilot-training}
% To estimate the efficiency of training with pilots across all methods, we consider a new transmission model, where a pilot block is transmitted before each data block as in Fig.~\ref{fig:pilots_eff_transmission}. The same number of data blocks is transmitted as in Subsection~\ref{subsec:synth_simulation_results} and Subsection~\ref{subsec:cost_simulation_results} for the \ac{mimo} cases, where $T_d = 50$ and $T_d = 40$, respectively. Now, we set the length of data blocks to constant 5000 bits in order to check adaptation over long blocks. No coding scheme is employed; Instead, we only train on the pilot blocks, whose size varies. Pilot blocks are immediately inserted into the buffer in the meta-training approach, as specified in Algorithm~\ref{alg:online-meta-learning}.  

% Moving to results, we consider the flat \ac{mimo} channels as above. Here, one may observe that our training approach is preferable to  the other approaches at most lengths, for the linear synthetic as well as the COST 2100 channel (Fig.~\ref{fig:pilots_efficiency_mimo}). We highlight that our method is able to better utilize the model-based architecture of the detector to it's maximum efficiency, compared to model-free architecture, exploiting the pilots for better performance and consistently lower error rates than the other compared methods.

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.67\textwidth,height=0.09\textheight]{fig/pilots_eff_transmission.png}
%     \caption{The new data transmission model with periodic transmission of pilots.}
%     \figSpace
%     \label{fig:pilots_eff_transmission}
% \end{figure*}

% \begin{figure*}[!t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/synth_pilots_efficiency_mimo.png}
%     \caption{Synthetic channel, ${\rm SNR} = 12$ dB.}
%     \label{fig:synth_pilots_efficiency_mimo}
%     \end{subfigure}
%     %
%     \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth,height=0.22\textheight]{fig/cost_pilots_efficiency_mimo.png}
%     \caption{COST 2100 channel, ${\rm SNR} = 14$ dB..}
%     \label{fig:cost_pilots_efficiency_mimo}
%     \end{subfigure}
%     %
%     \caption{SER vs. pilots size with $\Blklen = 96$.}
%     \label{fig:pilots_efficiency_mimo} 
%     \figSpace
% \end{figure*}


==> sections_v1/system_model.tex <==
\section{System Model}
\label{sec:Model}
\vspace{-0.1cm}

In the section, we describe the system model in Subsection~\ref{subsec:Channel}, and then formulate the communication protocol and the design problem in Subsections~\ref{subsec:Transmission} and \ref{subsec:Problem}, respectively. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth,height=0.1\textheight]{fig/transmission_model.png}
    \caption{Transmission model. The channel is constant in each block and  changes across blocks. }
    \figSpace
    \label{fig:transmission}
\end{figure*}

% \textcolor{red}{This section needs to be re-organized. Before describing the communication protocols, which is divided into blocks, I think we should introduce the block-wise varying channel model. Second, the detection scenario  in Subsec. \ref{subsec:Transmission} does not discuss detection; it explains the considered transmission protocol.  Finally, the formulated problem does not really capture the problem that we are trying to solve.
% \\
% So we should start with the generic channel model, and emphasize that the actual input-output relationship in \eqref{eqn:ChModel1} may be highly complex. We should also indicate that the variations in the channel between blocks are often not arbitrary and can be due to, e.g., movement of some of the communicating entities. We build on this property in two aspects of our solution - the fact that we train on one channel for to following one, and the modular training procedure. \\ 
% Then, we should proceed by describing the communication protocol, where you explain the division into pilots and data, and don't forget to clarify that coding includes both \ac{fec} and error detection - our solution relies on their existence. \\
% Finally, present the formulation of the problem, which should be what we are trying to solve. Now, we are not designing a symbol detection mechanism that imitates the MAP rule, we are proposing an algorithm which allows a \ac{dnn} aided receiver, whose input-output mapping is dictated by a parameter vector $\theta$, to adapt its parameters over time in order to continuously provide low error rates over the data blocks. 
% }

%-----------------------------------
%	Block-Fading Channel Model
%-----------------------------------
\vspace{-0.2cm}
\subsection{Channel Model}
\label{subsec:Channel}
\vspace{-0.1cm} 

We consider communication over casual finite-memory block-wise varying channels with multiple users. The channel output depends on the last $\Mem >0$ transmitted symbols, where $\Mem$ is the memory length. The channel is constant within a block of $\Blklen$ channel uses, which corresponds to the coherence duration of the channel. 

Let $\myVec{S}_{i,j}\in\mySet{S}^K$ be the symbol transmitted from constellation $\mySet{S}$ at the $i$th time instance, $i \in \{1,2,\ldots, \Blklen\}:= \Blkset$, of the $j$th block. Here, the constellation size is $|\mySet{S}|$ and $K$ denotes the number of symbols transmitted at each time instance, e.g., the number of users transmitting simultaneously in an uplink communications channel. Let $\hat{\myVec{u}}$ stand for the transmitted channel word, modulated into the above $\myVec{s}$.
The channel output is denoted by $\myY_{i,j}\in \mySet{Y}^N$, where $N$ represents the number of receive antennas, and is given by a stochastic function of the last $L$ transmitted symbols 
%$\myVec{S}_{i,j-\Mem+1},\ldots, \myVec{S}_{i,j}$.
$\myState_{i,j} := [\myVec{S}_{i-\Mem+1,j},\ldots, \myVec{S}_{i,j}]^T$.  
Specifically, by defining the $j$th transmitted block as $\myS_j := \{\myVec{S}_{i,j}\}_{i\in \Blkset}$ and its corresponding observations as $\myY_j:= \{\myY_{i,j}\}_{i\in \Blkset}$,  the conditional distribution of the channel output given its input satisfies   
\begin{equation}
	\label{eqn:ChModel1}
	P_{\myY_j | \myS_j}\left(\myVec{y}_j | \myVec{s}_j \right)  = 
	\prod\limits_{i\!=\!1}^{\Blklen}P_{\myY_{i,j} |\myState_{i,j}}\left(\myVec{y}_{i,j} |\mystate_{i,j}\right).  
\end{equation}
In \eqref{eqn:ChModel1}, the lower-case notations $\myVec{s}_j$, $\myVec{y}_{i,j}$, and $\myStateR_{i,j}$ represent the realizations of the \acp{rv} $\myS_j$, $\myY_{i,j}$, and $\myState_{i,j}$, respectively. We set $\myVec{S}_{i,j} \equiv \myVec{0}$ for $i<0$, i.e., we assume a guard interval of at least $\Mem-1$ time instances between blocks.

%Practical communication scenarios are highly complex; 

The input-output relationship in \eqref{eqn:ChModel1} describes a generic channel model with block-wise temporal variations. These  channel variations, i.e., changes between different values of the block index $j$, can often be attributed to some phenomena, e.g. a  movement  of one or several of the communicating entities. %Our two-stage training method is tailored for these complex scenarios, exploiting domain knowledge, whereas naive algorithms fail. 
We do not impose a specific model on the channel observed in each block, representing it by the generic conditional distribution in \eqref{eqn:ChModel1}, which can take a complex and possibly intractable form. Two important special cases of this channel model include:
\begin{enumerate}
    \item \emph{\ac{siso} Finite-Memory Channels}: The first type of channels considered in this work is the multipath \ac{siso} case; That is, we set $N=K=1$. 
    \item \emph{Flat \ac{mimo} Channels}: Another channel of interest is the memoryless ($L=1$) \ac{mimo} channel, where $N>1$ and $K>1$. Such settings specialize multi-user uplink \ac{mimo} systems, where $K$ is the number of single-antenna transmitters. 
\end{enumerate}




%-----------------------------------
%	Transmission
%-----------------------------------
\vspace{-0.2cm}
\subsection{Communication Protocol}
\label{subsec:Transmission}
\vspace{-0.1cm}  

We consider the scenario illustrated in Fig.~\ref{fig:transmission}, where a total of $T_p$ pilot blocks and $T_d$ information blocks are transmitted sequentially. That is, blocks indexed $j\in\{0,\ldots,T_p-1\}$ are known pilots, \SangwooCmt{transmitted in the training phase,}  while $j\in\{T_p,\ldots,T_p+T_d-1\}$ are information blocks \SangwooCmt{that compose the test phase}. The pilot blocks convey a known message, whereas the information blocks are unknown and are utilized to test the proposed schemes. Each information block, i.e., $\myVec{S}_j$ for $j\in\{T_p,\ldots,T_p+T_d-1\}$, is encoded into a total of $B$ symbols using both \ac{fec} coding and error detection codes. Error detection codes, such as cyclic redundancy check, allow the receiver to identify the presence of errors in the decoding procedure.

%-----------------------------------
%	Problem Formulation
%-----------------------------------
\vspace{-0.2cm}
\subsection{Problem Formulation}
\label{subsec:Problem}
\vspace{-0.1cm}  
We consider the problem of symbol detection in the generic channel model formulated in Subsection~\ref{subsec:Channel}. The fact that we do not impose a specific model of the channel, allowing its input-output relationship to take complex forms in each block, combined with the availability of data based on the protocol detailed in Subsection~\ref{subsec:Transmission}, motivate using \ac{dnn}-aided receivers. The core challenge in applying \ac{dnn}-aided receivers for the considered channel stems from its temporal variations. Our objective is thus to derive a training algorithm that aids \ac{dnn}-aided receivers in recovering the transmitted data from the channel outputs  $\{\myVec{Y}_j\}_{j=T_p}^{T_p+T_d-1}$. \SangwooCmt{The \ac{dnn}-aided receiver trains on the pilot blocks, and is tested on the transmitted information blocks.}

In particular, we let $\Weights$ denote the parameters of the \ac{dnn}-aided receiver, i.e., the weights of the neural network. These parameters dictate the receiver mapping, which, for a given $\Weights$, is denoted by $\hat{\myVec{s}}(\cdot; \Weights):\mySet{Y}^{N\times \Blklen } \mapsto \mySet{S}^{K\times \Blklen}$, i.e., $\hat{\myVec{s}}(\myVec{y}; \Weights)$ denotes the symbol block recovered\footnote{while the \ac{dnn}-aided receiver is formulated here as outputting symbol decisions, one can also adapt the formulation to soft (probabilistic) decisions. } by the receiver parameterized with $\Weights$ when applied to the channel output block $\myVec{y}$. By using the abbreviated symbol  $\hat{\myVec{s}}_j(\Weights)$ to denote the symbols detected based on the channel output of the $j$th block, with $\hat{\myVec{s}}_{i,j}(\Weights) \in \mySet{S}^K$ being its $i$th symbol, $i \in \Blkset$, our goal is to propose an algorithm that allows a DNN-aided receiver  to  continuously provide low error rates over the data blocks:
\begin{equation}
\label{eqn:ErrorRate}
	\mathop{\min}_{\Weights_j}\Big(\frac{1}{\Blklen}\sum_{i=1}^{\Blklen} \Pr\left( \hat{\myVec{s}}_{i,j}(\Weights_j) \neq \myVec{s}_{i,j} \right)\Big), \qquad j\in\{T_p,\ldots,T_p+T_d-1\}. 
\end{equation}
The parameter vector $\Weights$ in \eqref{eqn:ErrorRate} is allowed to change between blocks, namely, the \ac{dnn}-aided receiver can adapt its parameters over time, while \SangwooCmt{the pilot blocks are utilized to initialize $\Weights$.}

As our problem formulation does not impose a specific structure on the \ac{dnn}-aided receiver, we first consider an online adaptation mechanism that is agnostic of the structure of the \ac{dnn}-aided receiver, after which we show how one can further benefit when the \ac{dnn} has an interpretable modular architecture.
